An Approach and Benchmark to Detect Behavioral Changes of Commits in Continuous Integration

When a developer pushes a change to an application's codebase, a good practice is to have a test case specifying this behavioral change. Thanks to continuous integration (CI), the test is run on subsequent commits to check that they do no introduce a regression for that behavior. In this paper, we propose an approach that detects behavioral changes in commits. As input, it takes a program, its test suite, and a commit. Its output is a set of test methods that capture the behavioral difference between the pre-commit and post-commit versions of the program. We call our approach DCI (Detecting behavioral changes in CI). It works by generating variations of the existing test cases through (i) assertion amplification and (ii) a search-based exploration of the input space. We evaluate our approach on a curated set of 60 commits from 6 open source Java projects. To our knowledge, this is the first ever curated dataset of real-world behavioral changes. Our evaluation shows that DCI is able to generate test methods that detect behavioral changes. Our approach is fully automated and can be integrated into current development processes. The main limitations are that it targets unit tests and works on a relatively small fraction of commits. More specifically, DCI works on commits that have a unit test that already executes the modified code. In practice, from our benchmark projects, we found 15.29% of commits to meet the conditions required by DCI.

==> Autoref.tex <==
\usepackage{catoptions}
\makeatletter
\def\figureautorefname{figure}
\def\tableautorefname{table}
\def\Autoref#1{%
  \begingroup
  \edef\reserved@a{\cpttrimspaces{#1}}%
  \ifcsndefTF{r@#1}{%
    \xaftercsname{\expandafter\testreftype\@fourthoffive}
      {r@\reserved@a}.\\{#1}%
  }{%
    \ref{#1}%
  }%
  \endgroup
}
\def\testreftype#1.#2\\#3{%
  \ifcsndefTF{#1autorefname}{%
    \def\reserved@a##1##2\@nil{%
      \uppercase{\def\ref@name{##1}}%
      \csn@edef{#1autorefname}{\ref@name##2}%
      \autoref{#3}%
    }%
    \reserved@a#1\@nil
  }{%
    \autoref{#3}%
  }%
}
\makeatother

==> old-stuff/SECI.tex <==
%
%   JBSE
%
\subsection{Symbolic Execution for Change Detection}
\label{subsec:jbse}

Symbolic execution is one popular technique for change detection \cite{TillmannSymbc}. 

% How we use it as amplification
We adapt this technique for test amplification as follows.
First, for each test method, we generate a new version of the method in which we extract all the literals (int, long, boolean) and turn them into parameters for the method. In addition, all assertions are removed. Second, we execute this new version of the method symbolically. In turn, we collect a set of constraints, which we pass on to a SMT solver. The solver returns concrete values  that can be used as test inputs.
Eventually, one new test method per solution found by the solver. 
Since these new test methods do not include assertions, the third step of our amplification process runs \aampl on each of them.

\todo{put an algo}

\begin{lstlisting}[caption={Original test method to be amplified},label=lst:jbse:original_test,float,language=java,numbers=right] 
@Test
void testCompute() {
 Calculator calculator = new Calculator(23);
 int compute = calculator.compute(32, 42);
 assertEquals(1, compute);
}
\end{lstlisting}

Let us illustrate this amplification process with an example.  \autoref{lst:jbse:original_test} is an original manually written test.
In this original test method, there are 3 integers (excluding the one in the assertion). The extraction,  results in a new method that takes 3 integers as parameters and does not include any assertion, as in \autoref{lst:jbse:wrapped_test}.

\begin{lstlisting}[caption={Extracted parametrized test from the original test method},label=lst:jbse:wrapped_test,float,language=java,numbers=right] 
void parametrizedTestCompute(int param1, int param2, int param3) {
 Calculator calculator = new Calculator(param1);
 int compute = calculator.compute(param2, param3);
}
\end{lstlisting}

Then, we execute  this method symbolically. Each parameter is considered as a symbol. During this execution, we collect different constraint to execute different path. For instance, to trigger one of the specific path of the application, the values must satisfy the following constraint: 
$param1 \neq param2 \wedge param1 \neq param3 \wedge param2 > param3 \wedge param2 + 7 - 15 > param3$. The SMT solver finds a solution for this problem: $param1=0, param2=1, param3=-7$. Eventually, we replace each original literal by the new values to obtain an amplified test method in. Finally, we run \aampl and generate the test case displayed in \autoref{lst:jbse:amplified_test}.

\begin{lstlisting}[caption={Amplified test method obtained using the symbolic execution.},label=lst:jbse:amplified_test,float,language=java,numbers=right] 
@Test
void testCompute_SymbEx1() {
  Calculator calculator = new Calculator(0);
  int compute = calculator.compute(1, -7);
  assertEquals(7, compute);
}
\end{lstlisting}

==> old-stuff/case_studies.tex <==
%
%   CASE 1
%
\subsection{Case study: protostuff\#167}
\label{subsec:pr1}
The first pull request we consider as case study is in an open-source project called protostuff, which provides advanced serialization features for Java. It has 1485 commits, 14 contributors, 686 star gazers, and 70K lines of code.

The considered pull request is protostuff\#167\footnote{\url{https://github.com/protostuff/protostuff/pull/167}}, it modifies the \texttt{toString()} method of class \texttt{io.protostuff.ByteString}.  \autoref{fig:protostuff167} shows a screenshot of the pull request.
In this  pull request, the developers change the String representation of the \texttt{ByteString}s as follows: instead of using a plain String representation of the array of bytes, the representation is now a String that includes a hashcode of the \texttt{ByteString} and its size.
First, we make sure that this pull request contains a behavioral change, because it contains a new test case that fails on the \base version. We compute the graphical signature of the pull request of the \base test suite:

$$
TS\begin{pmatrix}BASE\\PR\end{pmatrix}
=
\begin{pmatrix}$\cmark$\\$\cmark$\end{pmatrix}
$$


\begin{figure}[!h]
\centering
\fbox{\includegraphics[width=0.45\textwidth]{changes_protostuff_167.png}}
\caption{Application change in pull request \href{https://github.com/protostuff/protostuff/pull/167}{protostuff\#167} in class ByteString.}
\label{fig:protostuff167}
\end{figure}

Now, we see whether a behavioral change detection technique is able to detect this modification.
For this, we apply both \aampl and \sbampl to the test \texttt{testCompareVsOther} of the test class \texttt{LowCopyProtobufOutputTest}.
The first task to do select test to be amplified: here the application change is in class \texttt{ByteString}, so we select the tests that use at least one method of class \texttt{ByteString}. The selected test is \texttt{testCompareVsOther}, whose an excerpt is shown in \autoref{lst:protostuff167:original_test}. In this test, the method wrap from class ByteString is used. Note that the potentially offending string literals are those of the developers.

\begin{lstlisting}[
caption={Original test method of protostuff to be amplified},
label=lst:protostuff167:original_test,
float,
language=java,
numbers=left
] 
void testCompareVsOther() {
    Bar testBar = new Bar(22,
        ByteString.wrap("fuck yo test".getBytes()),
        false
    );
    ... // assert later on
}
\end{lstlisting}

\begin{lstlisting}[
caption={New test method of protostuff obtained with \aampl},
label=lst:protostuff167:amplified_test,
float,
language=java,
numbers=right
] 
void testCompareVsOther_amplified() {
    Bar testBar = new Bar(22, 
        ByteString.wrap("fuck yo test".getBytes()),
        false
    );
    assertEquals(22, testBar.getSomeInt());
(*@\xmark@*)  assertEquals("fuck yo test", testBar.getSomeBytes().toString());     assertFalse(testBar.getSomeBoolean());
}
\end{lstlisting}

From this test, \aampl generates a new test case with 3 new assertions in 2.7 minutes: two \texttt{assertEquals} and one \texttt{assertFalse}, that are shown in  \autoref{lst:protostuff167:amplified_test}.
The second \texttt{assertEquals} in line 7 is the one that can detect the behavioral change: it captures the behavior of the \base branch in which the String representation of a \texttt{ByteString} is a direct translation of the \texttt{ByteString}'s content. This assertion passes on the \base branch and fails on the new behavior proposed in \head branch.

This is is success for \aampl: this automatically generated test is able to capture the behavioral change. \sbampl also captures this change, since it supersedes \aampl. As a result, the pull request signature is the expected one, the same test suite TS highlights the behavioral difference between the \base version and the pull request.:

$$
ATS\begin{pmatrix}BASE\\PR\end{pmatrix}
=
\begin{pmatrix}$\cmark$\\$\xmark$\end{pmatrix}
$$


%
%   CASE 2
%
\subsection{Case study: javapoet\#550}
\label{subsec:pr2}

The second chosen pull request is from a project named Javapoet. Javapoet is a library for generating Java source code. It has 755 commits, 62 contributors, has 7K lines of code and has been starred 5398 times. 
Pull request \href{https://github.com/square/javapoet/pull/550}{javapoet\#550}\footnote{\url{https://github.com/square/javapoet/pull/550}} add not-null checks in the constructor of the \texttt{Builder} class and in method \texttt{addModifiers}. 
When the given parameter is \texttt{null}, the program throws an exception with a specific message. 
In the pull request, the developers add information in the exception flow in order to ease debugging. The graphical signature of this pull request for the \base test suite is the following, which means that there is no test case that specifies the behavioral change:

$$
TS\begin{pmatrix}BASE\\PR\end{pmatrix}
=
\begin{pmatrix}$\cmark$\\$\cmark$\end{pmatrix}
$$

\begin{figure}[!h]
\centering
\fbox{\includegraphics[width=0.45\textwidth]{changes_javapoet_550.png}}
\caption{Proposed changes in pull request \href{https://github.com/square/javapoet/pull/550}{javapoet\#550}.}
\label{fig:javapoet550}
\end{figure}

We now see if behavioral techniques detection works on this pull request. We apply \aampl and \sbampl to the test method \textit{nullExceptionsAddition} of \texttt{MethodSpecTest}, shown in \autoref{lst:javapoet550:original_test}.
This test specifies that when the parameter of the method \texttt{addExceptions} is \texttt{null}, the program throw an exception with a specific message (call to method \texttt{hasMessage}). 

\begin{lstlisting}[
caption={Original test method of javapoet to be amplified},
label=lst:javapoet550:original_test,
float,
language=java,
numbers=left
] 
@Test 
void nullExceptionsAddition() {
    try {
      MethodSpec.methodBuilder("doSomething").addExceptions(null);
      fail();
    } catch (IllegalArgumentException expected) {
      assertThat(expected).hasMessage("exceptions == null");
    }
}
\end{lstlisting}

First, we apply \aampl and notice that \aampl does not succeed to detect the behavioral change.
Next, we apply \sbampl. For this pull request, \sbampl manages to produce a test that specifies the behavioral change in 20 minutes. It results with the amplified test method shown in \autoref{lst:javapoet550:amplified_test}.

\begin{lstlisting}[
caption={New test method of javapoet(\#550) obtained with \sbampl},
label=lst:javapoet550:amplified_test,
float,
language=java,
numbers=left
] 
@Test
void nullExceptionsAdditionlitString2_failAssert0() {
    try {
        try {
            MethodSpec.methodBuilder(null).addExceptions(null);
        } catch (IllegalArgumentException expected) {
        }
        fail("nullExceptionsAdditionlitString2 should have thrown NullPointerException");
    } catch (NullPointerException expected_1) {
(*@\xmark@*)        assertEquals(null, expected_1.getMessage());
    }
}
\end{lstlisting}

The amplification applied to obtain this valuable new test method is as follow: 
1) \sbampl replaces the literal string \texttt{"doSomething"} by a \texttt{null} value; 
2) \aampl executes the transformed test method
3) since the method now throws an exception with this new parameter, \aampl wraps the body with a try/catch block (to catch a \texttt{NullPointerException}). It adds a fail statement at the end of the body of the try, \ie it expects that the exception is thrown, and adds an assertion on the message of the exception. The message is null in this case, since the exception is generated by the JVM.

When executing this automatically generated test method on the \head branch, it fails, while it passes on the \base branch, which proves that the behavioral change has been specified. 
The \texttt{assertEquals(null, expected\_1.getMessage())} in Line 10, marked by \xmark, captures the behavioral changes since the message of the exception is no more null. Finally, the amplified test suite (ATS) has the correct test signature: 

$$
ATS\begin{pmatrix}BASE\\PR\end{pmatrix}
=
\begin{pmatrix}$\cmark$\\$\xmark$\end{pmatrix}
$$


%
%   CASE STUDY 3
%
\subsection{Case study: javapoet\#608}
\label{subsec:pr3}

The third and final case study of this paper is about pull request \href{https://github.com/square/javapoet/pull/608}{javapoet\#608}\footnote{\url{https://github.com/square/javapoet/pull/608}}, from the same project javapoet as the previous case study. As shown in \autoref{fig:javapoet608}, this pull request modifies the method \texttt{zeroWidthSpace} from the \texttt{LineWrapper} object. This method is responsible to insert a new line and to update the indentation level of a Java source file. The pull request aims at fixing the behavior as follows: if the current line has no indentation, \ie the \texttt{column} is equal to zero, the method should  directly return.
This pull request does not specify the behavioral change and consequently, the test signature is:

$$
TS\begin{pmatrix}BASE\\PR\end{pmatrix}
=
\begin{pmatrix}$\cmark$\\$\cmark$\end{pmatrix}
$$

\begin{figure}[!h]
\centering
\fbox{\includegraphics[width=0.45\textwidth]{changes_javapoet_608.png}}
\caption{Proposed changes in pull request \href{https://github.com/square/javapoet/pull/550}{javapoet\#608}.}
\label{fig:javapoet608}
\end{figure}


We apply \aampl and \sbampl on test method \texttt{wrapEmbeddedNewlines\_ZeroWidth} from \texttt{LineWrapperTest}, because they both invoke method \texttt{zeroWidthSpace}, shown in \autoref{lst:javapoet608:original_test}

\begin{lstlisting}[
caption={Original test method of javapoet to be amplified for \#608},
label=lst:javapoet608:original_test,
float,
language=java,
numbers=left
]
@Test
public void wrapEmbeddedNewlines_ZeroWidth() {
    StringBuffer out = new StringBuffer();
    LineWrapper lineWrapper = new LineWrapper(out, "  ", 10);
    lineWrapper.append("abcde");
    lineWrapper.zeroWidthSpace(2);
    lineWrapper.append("fghijk\nlmn");
    lineWrapper.append("opqrstuvwxy");
    lineWrapper.close();
    assertThat(out.toString()).isEqualTo("abcde\n    fghijk\nlmnopqrstuvwxy");
}
\end{lstlisting}

Only \sbampl succeeds to generate an amplified test method that detect the behavioral changes. This amplified test method is shown in \autoref{lst:javapoet608:amplified_test}.

\begin{lstlisting}[
caption={New test method of javapoet(\#550) obtained with \sbampl},
label=lst:javapoet608:amplified_test,
float,
language=java,
numbers=left
] 
@Test
public void wrapEmbeddedNewlines_ZeroWidth_rm147_rm598() {
    StringBuffer out = new StringBuffer();
    LineWrapper lineWrapper = new LineWrapper(out, "  ", 10);
    lineWrapper.zeroWidthSpace(2);
    lineWrapper.append("opqrstuvwxy");
    lineWrapper.close();
(*@\xmark@*)  assertEquals("\n    opqrstuvwxy", out.toString());
}
\end{lstlisting}


In 2.11 minutes \sbampl is successful in detecting the behavioral change, by applying the following transformations.
First, it removes both method calls on Lines 5 and 7. Then, it adds assertions on observable values of the variable \texttt{out}. It results with a single assertion, on line 8 marked by \xmark, which captures the behavioral  difference between the two versions of the program (he \base and the \head branches). After the \head changes, the expected value of \texttt{out.toString()} is "opqrstuvwxy" without new line character and indentation.
As expected, the test signature of the amplified test suite (ATS) shows that the behavioral change is now specified:
 
$$
ATS\begin{pmatrix}BASE\\PR\end{pmatrix}
=
\begin{pmatrix}$\cmark$\\$\xmark$\end{pmatrix}
$$

%
%   DISCUSSION 
%
\section{Discussion}
\label{sec:discussion}

\subsection{Applicability}

Now we discuss about the perfect use case of behavioral change detection.
Assume that 
a developer proposes changes through a pull request, however, the pull request is poorly tested.
In the pull request, there are no tests or the provided tests do not sufficiently specify the behavioral changes.
In this case, one applies behavioral change detection in order to generate a test method that specifies the behavioral changes intended by the developer.
In this way, the developers who review the pull request have a clear understanding of the proposed changes, assisted by a specific test method that shows the behavioral changes.

\emph{Summary: Behavioral change detection is particularly applicable in communities where not all developers know how to well test changes.}


\subsection{Limitations}


% AAMPL
\aampl is a simple approach, which fits into
Andreas Zeller's of simplicity for software engineering\footnote{Keynote ICSE18: \url{https://www.icse2018.org/getImage/orig/ICSE+2018+Keynote+Zeller.pdf}}.
However, to our experience, the behavioral changes detectable by \aampl, alone, are a small subset of all possible behavioral changes. 
\aampl requires that the pull request changes have an impact visible through \emph{getters} (see \autoref{subsec:aampl}). 
However, in many cases, it is required to do more than adding calls to getters. 

% SBAMPL
On the contrary, \sbampl is able to change the program state in order to trigger the new behavior.
Indeed, our first observations on the effectiveness of \sbampl seem promising.
Yet, we note that \sbampl is not mature enough to be integrated into the continuous integration process.
In particular, the search space of \sbampl is too large to be exhaustively explored, and thus it is too time consuming with respect to the available continuous integration resources.

\emph{Summary: \aampl is fast but too weak, \sbampl is effective but too time consuming. This calls for more research on behavioral change detection in large Java software.}


% -----------------------
%  THREATS TO VALIDATION
% -----------------------

\subsection{Threats to validity}

\paragraph{Internal threats}

We develop a prototype for each approach, and we do not exclude the presence of bugs in the code, which is a threat to the internal validity. Yet, for lying down solid foundations in this research area, all the code and the results are available online\footnote{\url{https://github.com/STAMP-project/Ex2Amplifier-experiments.git}} under the LGPL v3.0 license.

\paragraph{External threats}

%\todo{I have two problems with "external validty" 1) it's not about external validity 2) it contradicts with the fact that the initial signature of all pull request is green-green. What am I missing?}

We verify that each studied pull request actually introduces a behavioral change. This verification has been done in two steps:
1) each pull request comes with a new unit test method. We execute the new test method on the \base branch. Since the new test methods was failing for the three case studies on the \base branch, it means that the pull request carries a behavioral change, \ie for the same input, the input of the test method, the observed output state of the program is different, the oracle part is passing or failing. According to our definition of behavioral change (see \autoref{subsec:behavioral:change}), the chosen pull request introduces a new behavior;
2) we manually verify the changes to confirm the first check.

==> old-stuff/concolic-exec-for-behavioral-change-detection.tex <==


%
%   CATG
%
\subsection{Concolic Execution}
\label{subsec:catg}
% Which tool
Concolic execution refers to the idea to mix concrete execution and symbolic execution \cite{}. 

%How it works?
\catg is a test generator based on concolic execution. It takes as inputs a \java standard \emph{main} method. It requires calls to specific method of the \catg framework to consider variables as symbol. For instance, in a `main` there is a local variable as follow: \texttt{int x = 0;}. \catg requires that this statement is transformed into: \texttt{int x = CATG.readInt(0);}. In this way, \catg collect both information: \texttt{x} can be symbolized, and one of its concrete value is \texttt{0}. \catg produces as output, files that contains values for each marked variable. Each file contains a set of values that trigger a specific path in the program.

% How we us it as amplification
To turn \catg into an amplification process, we need to transform test methods to be amplified into \java standard \emph{main} method, such as been done for \jbse. In addition to this, all the literals in the test method is transformed into local variables, initialized with the correct method call, according to the type, of the \catg framework. Not as \jbse, \catg produces directly usable values. For each files produces by \catg, we replace literals by the corresponding values to obtain one amplified test method per files.

Such as \jbse, \catg provides only new inputs, we also use \aampl on amplified test method to obtain new assertions.



==> old-stuff/notes.tex <==
\todo{read and select the relevant ones + chech citers}

1. Achieving traceability in large scale continuous integration and delivery deployment, usage and validation of the eiffel framework. Empirical Software Engineering, 2017

2. Cinders - The continuous integration and delivery architecture framework. Information \& Software Technology, 2017

%
% SIZE OF COMPANIES ETC, not really relevant.
%
3. The continuity of continuous integration - Correlations and consequences. Journal of Systems and Software, 2017

4. Reinforcement learning for automatic test case prioritization and selection in continuous integration. ISSTA, 2017


%
%   STUDY Of TRNASITION TO USING TRAVIS CI
%
5. The impact of continuous integration on other software development practices - a large-scale empirical study. ASE, 2017

6. TravisTorrent - synthesizing Travis CI and GitHub for full-stack research on continuous integration. MSR, 2017

7. An empirical study of activity, popularity, size, testing, and stability in continuous integration. MSR, 2017

8. The impact of the adoption of continuous integration on developer attraction and retention. MSR, 2017

9. Insights into continuous integration build failures. MSR, 2017

10. An empirical study of the personnel overhead of continuous integration. MSR, 2017

11. On the interplay between non-functional requirements and builds on continuous integration. MSR, 2017

12. Impact of continuous integration on code reviews. MSR, 2017

%
%   Others errors than test failures in CI
%
13. An empirical analysis of build failures in the continuous integration workflows of Java-based open-source software. MSR, 2017

14. How open source projects use static code analysis tools in continuous integration pipelines. MSR, 2017

15. Trade-offs in continuous integration - assurance, security, and flexibility. ESEC/SIGSOFT FSE, 2017

16. Measuring the cost of regression testing in practice - a study of Java projects using continuous integration. ESEC/SIGSOFT FSE, 2017

17. Industry application of continuous integration modeling - a multiple-case study. ICSE, 2016

% short paper of Hilton:2016:UsageCI
19. Understanding and improving continuous integration. SIGSOFT FSE, 2016

An empirical comparison of automated generation and classification techniques for object-oriented unit testing

Evacon: A framework for integrating evolutionary and concolic testing for object-oriented programs

Automated Regression Testing using Symbolic Execution

==> old-stuff/old-experiments.tex <==
%
%   XP PROTOCOL
%
\section{Experimental protocol}
\label{sec:protocol}

\todo{Benoit Martin: go over A, B and C}
We aim at revealing which of the techniques introduced in \autoref{sec:compared_techniques} would be the best at improving the behavioral change detection capacities of a test suite. We also want to balance this improvement of the test suite with  the time required to obtain this improvement.

A pull request provides  two versions of the same program. In our experiments, we consider only pull requests that actually introduce  a behavioral change.

The process for the comparison is as follows: 
For a given pull request, we select test methods to be amplified.
Then, we apply the tool to amplify the selected test methods. It results with a set of amplified test methods, a better version of the existing one.
Eventually, we execute the amplified test methods on the other version of the program. If any amplified test methods fail, it means that the tool is able to produce test methods that are able to capture the behavioral differences between the two versions of the program.

This process is applied using both version of the program: the \base branch and the \head branch as ground truth, see \autoref{subsec:aampl} for more information. 

%
%   PROJECT SELECTION
%
\subsection{Project selection criterion}

We use a subset of the projects from a dataset of another paper\cite{DSpot}. This dataset is based on activities of the community, the quality of the code and of the test code and development process, \ie pull request based development.

%
%   PR SELECTION
%
\subsection{Pull request Selection Criteria}

For each considered project, we aim at selecting at least 5 and at most 10 pull requests. 
The selection is made according to the following criteria: 
1) the pull-request has been merged; 
2) the merged branch is still available (not deleted on \gh);
3) the pull request modifies the source code (\ie we exclude pull-requests with test code modification only, or pull-requests with configuration and documentation change only).
% if we are able to explain this better we can put it again
% 4) The modified methods are present in both version., \ie if the pull request add a new feature for users, that is not used nor tested, we do not consider it (\eg see \url{https://github.com/protostuff/protostuff/pull/211/files}), in this case, the project would need a generator of test and not an amplifier.

For the \nbProjects considered, this results in \nbPullRequests.

% SANITY: 
% Javapoet 529 OK

% JSOUP 1038 KO
% JSOUP 931 OK
% JSOUP 881 OK (kind of, for me, when a redirect happen, the body is null on the PR BRANCH but not null on the BASE branch)

% MYBATIS-3 1149 KO The detection is due to the modification of the visibility, it might be included in behavioral changes
% MYBATIS-3 1110 OK

% PROTOSTUFF 201 OK
% PROTOSTUFF 185 OK
% PROTOSTUFF 182 OK

\newcommand{\nbAlphaPR}{9\xspace}

For each pull request, we compute the graphical signature. It results with \nbAlphaPR $\alpha$ signatures over \nbPullRequests. For them, we manually verify that a behavioral changes has been introduced. 

%\todo{discuss about the two cases Jsoup\#1038 and mybatis-3\#1149}

%
%   TEST SELECTION
%
\subsection{Test case selection criterion}
\label{subsec:test_case_selection}

We select test cases to be amplified according to the diff between the base branch\footnote{at the time of the pull request} and the pull request branch.

This is done as follow: 
1) we use the command line \emph{git diff} to collect the diff between the two branches, \base and \head;
2) we collect the list of all modified files thanks to the diff;
3) we compute the list of modified test methods;
4) we compute the list of modified application methods;
5) we select modified application methods that are directly called in test methods, \ie their body have an invocation to a modified application method.

If this fails to identify test methods, we use the following alternative strategy:
we take all test methods of test classes whose name is composed of the modified application file prefixed or suffixed  with "Test" at the begin or at the end.
For instance, if \emph{my.package.MyClass} has been modified, we select all test methods of \emph{my.package.TestMyClass} and \emph{my.package.MyClassTest} for being amplified.

\subsection{Research questions}

Our study aims at answering to the following research questions:

% 
%  Research question
% 
\begin{itemize}
\item \RQ{1}{What proportion of pull-requests can be assessed with behavioral change analysis?}
%\item \RQ{2}{How does symbolic execution compare to a search-based method to improve tests in pull requests?}
\item \RQ{2}{To what extent is the execution time of amplification acceptable for pull-request based feedback?}
\item \RQ{3}{How do the amplified tests detect the behavioral changed according to a qualitative manual analysis?}
\end{itemize}

To answer to RQ$_{1}$, we use the following protocol: 
1) we take pull request one by one;
2) we select tests to be amplified according to the criteria (see \autoref{subsec:test_case_selection});
3) we amplify the tests using first the \base branch;
4) if any amplified tests is generated, we execute them on the \head branch;
5) if any of amplified tests fail on the the \head branch, we select them since they are able to identify a behavioral changes;

This protocol result with a set of amplified test that pass on the \base branch, but fail on the \head branch.
We compute the percentage of the pull request for which each techniques has been able to detect the behavioral change over the overall pull request, \ie \nbPullRequests.

%To answer to RQ$_{2}$, we compare the number of pull request on which \aampl, \seci and \iampl are able to detect the behavioral change, \ie able to amplified test methods that pass on the \base branch but fail on the \head branch. The more there are pull requests, the better is considered the approach to capture behavioral changes.

To answer to RQ$_{2}$, we compare the execution time of \aampl and \iampl. We compute the median execution time of each approach. The faster the process is executed, the better it is. In pull request based development, the time to get feedback is crucial, since developer cannot wait a day before getting merge its changes. This is why, we consider this aspect as much as we consider the effectiveness of the techniques to detect behavioral changes.

To answer to RQ$_{3}$, we manually analyze amplified tests that are able to detect a behavioral changes between the two version. To select which amplified test we analyze, we use the following criteria: we take for each approach the pull request on which the approach produces the maximum number of amplified test methods that detect the behavioral changes in the minimum of time execution. In other word, we take the result of the pull request that have the higher ratio $\frac{\# Success amplified tests}{Time}$. Or we take pull request for which every approaches are able to detect the behavioral change.

% -----------------------
%  Experimental Result
% -----------------------
\section{Experimental Result}

\input{table.tex}

Result are summarized in \autoref{tab:overall-result}.
The first column in the same of the project.
The second, the third and the fourth are respectively the unique ID of the considered pull request, the number of test methods selected to be amplified, and the number of line of code of the project, computed with the command line \texttt{cloc}.
The fifth is the graphical signature of the pull request see \autoref{subsubsec:sigpr}.
Then, there are three meta-column, for each techniques: \aampl and \iampl.
In the meta-column, the first column, the second and the third are respecitvely the number of test methods that could be obtained with the approach, the number of success, \ie the number of test methods that pass on the \base branch but fail on the \head branch and the execution time of the approach, in second (suffixed by 's') or minute (suffixed by 'm').

In the table, the yellow cells highlight pull request for which the approach has been able to amplify test methods, \ie the first column of the meta-columns $\#Amplified > 0$.
The green cells highlight pull request for which the approach has been able to obtain an amplified test method that detect the behavioral changes, \ie the second column of the meta-columns $\#Success > 0$.

%
%   RQ1
%
\RQ{1}{What proportion of pull-requests can be assessed with behavioral change analysis?}

In the table we observe the result for each approach. 
The absolute number of success of amplification for each approach are \TODO{29}, \TODO{9} and \TODO{26} over the \nbPullRequests pull requests for respectively \aampl and \iampl.
The absolute number of success of detection for each approach are \TODO{10}, \TODO{0} and \TODO{7} over the \nbPullRequests pull requests for respectively \aampl, \seci and \iampl.
This gives the following percentage: \aampl is able to detect \TODO{27}\% overall the pull request, \seci \TODO{0}\% and \iampl \TODO{19}\%.

The three techniques are able to amplify the tests.

\begin{mdframed}
\textbf{Answer}: Overall, the three approaches assess \TODO{30}\% of the \nbPullRequests behavioral changes.
\end{mdframed}

%
%   RQ2
%
%\RQ{2}{How does symbolic execution compare to a search-based method to improve tests in pull requests?}

%
%   RQ3
%
\RQ{2}{To what extent is the execution time of amplification acceptable for pull-request based feedback?}
The median of execution times \TODO{8s}, \TODO{8s} and \TODO{6m} for respectively \aampl, \seci and \iampl. The execution time of \aampl and \seci are relatively acceptable, while \iampl takes too much time to be executed in real life scenario. This is due to the fact that \aampl and \seci are applied only one time, while \iampl is applied three time. Also, \aampl and \seci do not produce a large number of amplified test methods because the search space is considerably small compared to the search space of \iampl. 

\begin{mdframed}
\textbf{Answer}: The execution time are respectively \todo{8s}, \TODO{8s} and \todo{6m} for \aampl, \seci and \iampl. The execution time of \aampl and \seci is acceptable, and their implementation inside the CI is realistic, while \iampl needs improvement.
\end{mdframed}

%
%   RQ4
%
\RQ{3}{How do the amplified tests detect the behavioral changed according to a qualitative manual analysis?}

\TODO{Analyze manually two amplified test 1 AAMPl and 1 SBAMPL}


==> old-stuff/old-protocol.tex <==

\subsection{Protocol}
\label{subsec:protocol}

Our protocol is as follows: 1) we select real pull requests from mature open-source projects 2) we apply behavioral change detection on the \base branch and 3) we discuss to what extent  behavioral change detection is successful.

\subsubsection{Project selection}
We consider projects from a dataset of another paper\cite{DSpotarXiv}. This dataset is composed of open-source projects with an active community, with high quality standards and based on pull request based development. In this paper, we consider two such projects: \emph{protostuff/protostuff}\footnote{https://github.com/protostuff/protostuff.git} and \emph{square/javapoet}\footnote{https://github.com/square/javapoet.git}.

\subsubsection{Pull request selection}
For each considered project, the selection of pull request is made according to the following criteria: 
1) the pull request has been merged; 
2) the pull request modifies the source code (\ie we exclude pull requests with test code modification only, or pull requests with configuration and documentation change only).

\subsubsection{Test method selection}

We select test cases to be amplified according to the diff between the \base branch\footnote{at the time of the pull request} and the \head branch.

This is done as follow: 
1) we use the command line \emph{git diff} to collect the diff between the two branches, \base and \head;
2) we collect the list of all modified files thanks to the diff;
3) we compute the list of modified test methods;
4) we compute the list of modified application methods;
5) we select modified test methods that call modified application method.

If this fails to identify test methods, we use the following alternative strategy:
we take all test methods of test classes whose name is composed of the modified application file prefixed or suffixed  with ``Test'' at the begin or at the end.
For instance, if \emph{my.package.MyClass} has been modified, we select all test methods of \emph{my.package.TestMyClass} and \emph{my.package.MyClassTest} for being amplified.



==> old-stuff/old-rw.tex <==
\subsection{Behavioral change detection}

%
%   BEHAVIORAL CHANGE DETECTION RW
%

Tillmann \etal~\cite{TillmannSymbc} exploits parametrized tests and symbolic execution to improve the coverage of programs. Their idea is that unit test methods can be generalized into parametrized tests, i.e. test that takes parameters. Then, for each set of parameters, the parametrized tests are instantiated and execute a specific portion of the code. They extract the parameters and transform them into rules, thanks to symbolic execution. Then, they use SMT solvers to generate values and obtain a high coverage. They evaluate there approach on a small benchmark of C\# classes and show that their approach can reveal bugs.
They successfully applied their approach on non-trivial classes and yet, not on real project like we do, by using open-source projects from \gh.



%
%  CI AND PR
%

\subsection{Continuous Integration}

Hilton \etal~\cite{Hilton:2016:UsageCI} conduct a study on the usage, costs and benefits of Continuous Integration. To do this, they use three complementary sources:  34,544 open-source projects from \gh, (ii) 1,529,291 builds from Travis, and (iii) they surveyed 442 engineers. Their findings are as follow: open-source project on \gh that use CI release twice more often, accept pull request faster and developers seem to be less worried about breaking existing features. Also, 70\% of the most popular project on \gh use heavily continuous integration.
This shows that the usage of continuous integration services such as Travis is widely used and became the trend. Our behavioral detection techniques is pluggable in the continuous integration.

Zampetti \etal~\cite{static:analysis:in:ci} investigate the usage of Automated Static Code Analysis Tools (ASCAT) in continuous integration. More precisely, they investigate which tools are used in the CI of open-source projects.
There investigation is done on 20 popular projects on \gh. According to their findings, coding guidelines is the most used tools in CI of open-source project. They also warn developers about heavy or improperly  usage of ASCAT like application specific errors or misconfiguration, which can produce a lot of false positive and thus slow down the continuous integration and the development process.
The warnings about the static analysis apply to our approach, it must not slow down the development process, however it needs further works.
%\todo{c'est un peu nul, j'avoue}

Spieker \etal~\cite{Spieker:RL:selection} elaborate a new approach for test case prioritization and selection in continuous integration. Their approach is based on reinforcement learning. They 1) show that test cases prioritization and selection can be modeled as a reinforcement learning problem using the history of  builds; 2) implement the approach in a tool; 3) apply their implementation over one year.
Spieker \etal aims at prioritazing and selecting test cases according to a changes, inside the continuous integration, while we aim at increasing the ability to detect behavioral changes of the test suite. The two approach could be combined to offer a powerful approach which would be effective and efficient.

%\todo{what's the link with CI? Here, the benchmark is done in the CI. The idea and the link is to talk about the portability of the behavioral changes detection techniques.}
Waller \etal~\cite{Waller:2015:IPB:2735399.2735416} study the portability of performance test to continuous integration. The idea is to automate the most steps of verification, but without impacting the time to feedback. To do this, they measure the performance overhead of the Kieker\cite{vanHoorn:2012:KFA:2188286.2188326} framework. The Kieker framework monitors the application-level performance. The framework as instrumentation to collect data and monitors and plugins to process them afterwards. Waller \etal developed a micro-benchmark, called MooBench, to monitor different kind of overhead of monitoring systems. 
They performed a pre evaluation using jenkins. They showed that Kieker has little variation between runs (every night runs) and claim that the performance test could and must be integrated in the CI, early as possible in the development of Software.
In our case, we do not target performance issue, but rather behavioral changed detection. However, the questions remains valid for our approach, it is possible to integrate it in the continuous integration, without breaking the development cycles? Our premise evaluation and case studies shows that \aampl is relatively usable in the CI, while \sbampl requires time execution reduction before genuinely used in the CI.

==> old-stuff/old-text.tex <==



pull request development \cite{Arie} is perfectly compatible with continuous integration: at each pull request, the CI service executes the code and tests of the pull request. Each time the pull request's author updates the pull request, for example after a code review, the CI service re-runs the tests.
To minimize the introduction of bugs, lead developers wait for the results of continuous integration before merging pull requests into the code base \cite{pr:based:dvlpp}.




in the context of pull request development. We propose two novel techniques that can be integrated in pull request development to  automatically detect behavioral changes. Those techniques are test amplification techniques \cite{survey:amplification}, which means that they modify existing tests in order to capture the behavioral change. 
Those two techniques are called \aampl and \sbampl, that we now shortly describe
\begin{itemize}
\item  \aampl stands for assertion amplification, and is grounded in the idea of adding the maximum number of assertions to existing test cases, based on the exhaustive exploration of public getter methods. This results in a tight specification of the behavior triggered in a test case. 
\item \sbampl stands for search-based amplification, it applies transformation operators to test cases in a search-based manner to trigger new behaviors. It can be seen as \textit{search-based testing} in the context of continuous integration.
\end{itemize}


We evaluate the two techniques on three detailed case studies of real pull requests from \gh. Using a systematic selection criteria, we execute \aampl and \sbampl on those three pull requests. We show that the approaches to detect behavioral changes have the potential to synthesize test cases that detect the behavioral changes. While the results are promising, they also reveal key challenges, either in applicability for \aampl, or in performance for \sbampl.







\footnote{\url{https://github.com/apache/commons-lang/commit/50ce8c4}}: This commit update the latest version of java, 11, handled by the project.
\autoref{fig:ampl_commons-lang} shows the amplified test obtained by DCI.
The test method \texttt{testGetJavaVersion} of JavaVersionTest has been used as seed for the amplification, and the resulting test contains 29 assertions. 
The assertion detecting the behavioral changes compare "JavaVersion.get("11")" to "1.8". In fact, "JavaVersion.get("11")" returns the latest supported version of Java, which 1.8 in the pre-commit version of the version.

\begin{figure}[h]
\centering
\fbox{\includegraphics[width=.95\linewidth]{img/amplified/amplified_commons-lang.png}}
\caption{Test generated by DCI that detects the behavioral change of \textsc{50ce8c4} in commons-lang.}
\label{fig:ampl_commons-lang}
\end{figure}

Let's have look to the human test in \autoref{fig:diff_commons-lang}. In this test, the developer update the latest version supported and a new assertion.

\begin{figure}[h]
\centering
\fbox{\includegraphics[width=.95\linewidth]{img/diff/diff_commons-lang.png}}
\caption{Provided test by the developer for \textsc{50ce8c4} of commons-lang.}
\label{fig:diff_commons-lang}
\end{figure}

DCI has been able to detect this behavioral change but the initial structure of the seed test method has been modified during the process. 





JSOUP Case study
\footnote{\url{https://github.com/jhy/jsoup/commit/426ffe7}}: this commit update the behavior of both methods \texttt{previousElementSiblings} and \texttt{nextElementSiblings}.
The amplified test is shown in \autoref{fig:ampl_jsoup}, it has been generated using \texttt{testPreviousElementSiblings} from ElementsTest.
It contains 60 assertions and capture the behavioral change when it compares the content of the first sibling.

\begin{figure}[h]
\centering
\fbox{\includegraphics[width=.95\linewidth]{img/amplified/amplified_jsoup.png}}
\caption{Test generated by DCI that detects the behavioral change of \textsc{426ffe7} of Jsoup.}
\label{fig:ampl_jsoup}
\end{figure}

We focus now the human test shown in \autoref{fig:diff_jsoup}.
The developer made twice the same change in two different test.
This modification remove an expected exception, and assert that the returned list of siblings is empty.

\begin{figure}[h]
\centering
\fbox{\includegraphics[width=.95\linewidth]{img/diff/diff_jsoup.png}}
\caption{Provided test by the developer for \textsc{426ffe7} of jsoup.}
\label{fig:diff_gson}
\end{figure}

\TODO{...}




==> old-stuff/old_background.tex <==
In this paper, we study two techniques to improve the ability of test suites to detect behavioral changes.
We focus on projects that follow a development process based on pull requests \cite{gousios2014exploratory}. 

%
%   PR & CI
%
\subsection{Pull request based Development \& Integration}

Our study considers software development processes based on pull requests (PR). On \gh, a pull request is a way for developers to propose their changes to the community of a given project. The pull request is composed of changes to the code, either source or test code, and has a title and a description. 
When a developer submits a PR, she creates a branch of the project that contains the proposed change. We call this branch the \head branch. The base version in which the developer wishes to merge her PR is called \base branch.

Before merging the \head into the \base, the PR goes through a two-fold review process: 
1) The continuous integration process (PR) is triggered. The PR automatically runs the test suites to detect the presence of regression bugs, \ie, behavioral changes introduced by the PR that impact the correctness of the program. However, the PR may fail to spot regression bugs if the test suite is too weak.
2) other developers look at the proposed changes and can either accept them or discuss their substance and form.

% example
\subsubsection{Pull request example}

Figure \ref{fig:example_pr_javapoet} displays a screenshot of a pull request on \emph{javapoet} \footnote{\url{https://github.com/square/javapoet/pull/608/files}}:

\begin{figure}[!h]
\centering
\fbox{\includegraphics[scale=0.25]{diff.png}}
\caption{Screenshot of a real pull request on \gh}
\label{fig:example_pr_javapoet}
\end{figure}

We can see the title of the pull request and the diff between the \base branch and the \head branch, which is one addition and four deletions to the source code.
We see the current state of the pull request, ``merged'', which means that the changes have been accepted and added to the \base branch.

% graphical
\subsubsection{Graphical signature of a pull request}
\label{subsubsec:sigpr}

We define a graphical signature for a pull request as the column-vector that summarizes the execution of a test suite on two versions of a program. 
The vector contains markers \cmark and \xmark. The \cmark means that the entire test suite passes, and the \xmark means that one or more tests fail.
Each row is two version of the same program, \base and \head branches.

With a strong test suite, we would have a column-vector identical to the following one
\begin{tabular}{c|c}
& Status \\
\hline
\base & \multirow{2}{*}{$\begin{pmatrix}$ \cmark $\\$ \xmark$\end{pmatrix}$} \\
\head & \\
\end{tabular}

%in~\autoref{tab:graph_sig_pr}.

A test suite in a pull request should identify behavioral changes. For example, ideally $TS$ would pass on \base but fail on \head because it detects and does not accept the behavioral change.
The \base test suite, $TS$, passes on the \base branch, but fails on the \head branch.
This means that the test suite specifies enough behavior to detect the difference between the two versions. In this case, \emph{we say the test suite detects a behavioral change.}
%
%   Behavioral Change
%
\subsection{Behavioral Change}
\label{subsec:behavioral:change}

We define behavioral changes as modifications in the source code that imply a new state of the program for the same inputs.
Considering the two branches \base and \head and the test suite $TS$ that exercises a set of inputs $I$, the PR introduces a behavioral change if the execution of $TS$ exhibits two different sets of states $S$ and $S'$, for respectively the \base branch and the \head branch.

%
%   Behavioral Change Detection
%
\subsection{Behavioral Change Detection}
\label{subsec:behavioral:change:detection}

We define behavioral change detection as the ability of a test suite to distinguish two versions of the same program. We approximate this detection by the fact that the test suite passes on a given version but fails on the other, \ie the verified states of the two versions of the same program, \base branch and \head branch are different.

In this paper, we aim at enhancing the ability of a test suite to detect behavioral changes.
To do this, we use test suite amplification because it exploits the existing test suite. Starting from high quality test methods will lead to better result rather than starting from scratch.
This is why, we modify each techniques to make them test suite amplification, \ie a process that automatically processes the program and the existing test suite in order to generate a better version of the test suite.

Based on the graphical signature introduced previously, we aim for the following improvement:

$$
TS\begin{pmatrix}BASE\\PR\end{pmatrix}
=
\begin{pmatrix}$\cmark$\\$\xmark$\end{pmatrix}
$$

%We define three patterns of graphical signature for any \head, as follows:
%1) all the tests pass on all versions;
%2) the test of the \head branch do not pass on the \base branch, \ie the \head contains a test that detect the behavioral change(s);
%and 3) the test of \base branch does not pass on the \head branch nor the test of the \head branch pass on the \base branch.
%The three patterns are summarized in \autoref{tab:graph_sign_pattern} .

%\begin{table}[h]
%\caption{Graphical signature patterns}
%\centering
%\begin{tabular}{c|c|c}
%$\begin{pmatrix}$\cmark$\\$ \cmark $\end{pmatrix}$&
%$\begin{pmatrix}$\cmark $\\$ \xmark $\end{pmatrix}$&
%$\begin{pmatrix}$\xmark $\\$ \cmark $\end{pmatrix}$\\
%$\alpha$&$\beta$&$\zeta$
%\end{tabular}
%\label{tab:graph_sign_pattern}
%\end{table}

% test vector
% $$
% TS\begin{pmatrix}BASE\\PR\end{pmatrix}
% =
% \begin{pmatrix}$\cmark$\\$\xmark$\end{pmatrix}
% $$

==> old-stuff/selection.tex <==
%
%   select
%
In this paper, we aim to amplify test methods to obtain new test methods that pass on the \base branch but fail on the \head branch. To do this, we use a specific implementation of the method $select()$, in Algorithm \autoref{algo:select}. For each $Test$ in the amplified test suite $ATS$ (Line 2), it executes $Test$ on the \head branch $P'$ (Line 3). If $Test$ fails, \ie $result.isFailing()$ is true (Line 4), then it adds $Test$ to the set of selected amplified test methods(Line 5).

\begin{algorithm}[h]
\begin{algorithmic}[1]
\REQUIRE{Amplified Test Suite $ATS$}
\REQUIRE{Program $P'$}
\ENSURE{Selected Amplified Test Suite $SATS$}
\STATE{$SATS \leftarrow \emptyset$}
\FOR{$Test$ in $ATS$}
    \STATE{$result \leftarrow execute(Test, P')$}
    \IF{$result.isFailing()$}
        \STATE{$SATS.add(Test)$}
    \ENDIF
\ENDFOR
\RETURN $SATS$
\end{algorithmic}
\caption{Selection of amplified test methods for behavioral changes detection.}
\label{algo:select}
\end{algorithm}

==> old-stuff/table-content.old.tex <==
& id  &  date  &  \#Test & SizeDiff{\color{ForestGreen}{+\xspace}} / {\color{red}{-\xspace}} &  Cov  &  \#SelectedTest  &  \#Aampl Tests  &  Success  &  Time(min)  &  \#Iampl Tests  &  Success  &  Time(min)\\
\hline
\multirow{11}{*}{\rotvertical{commons-io}}
&  c6b8a38  &  6/12/18  &  1348 &  {\color{ForestGreen}{104\xspace}} / {\color{red}{3\xspace}}  &  100.0  &  3  &  0  &  \xmark  &  0  &  0  &  \xmark  &  5\\
&  2736b6f  &  12/21/17  &  1343 &  {\color{ForestGreen}{164\xspace}} / {\color{red}{1\xspace}}  &  85.45  &  8  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  a4705cc  &  4/29/18  &  1328 &  {\color{ForestGreen}{37\xspace}} / {\color{red}{0\xspace}}  &  100.0  &  2  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  f00d97a  &  5/2/17  &  1316 &  {\color{ForestGreen}{244\xspace}} / {\color{red}{25\xspace}}  &  93.33  &  2  &  2  &  \cmark  &  0  &  178  &  \cmark  &  2\\
&  3378280  &  4/25/17  &  1309 &  {\color{ForestGreen}{5\xspace}} / {\color{red}{5\xspace}}  &  100.0  &  1  &  1  &  \cmark  &  0  &  114  &  \cmark  &  1\\
&  703228a  &  12/2/16  &  1309 &  {\color{ForestGreen}{6\xspace}} / {\color{red}{0\xspace}}  &  100.0  &  8  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  a7bd568  &  9/24/16  &  1163 &  {\color{ForestGreen}{91\xspace}} / {\color{red}{83\xspace}}  &  100.0  &  8  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  81210eb  &  6/2/16  &  1160 &  {\color{ForestGreen}{10\xspace}} / {\color{red}{2\xspace}}  &  100.0  &  1  &  0  &  \xmark  &  0  &  2  &  \cmark  &  0\\
&  57f493a  &  11/19/15  &  1153 &  {\color{ForestGreen}{15\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  8  &  0  &  \xmark  &  0  &  0  &  \xmark  &  1\\
&  e76397c  &  11/12/15  &  1125 &  {\color{ForestGreen}{9\xspace}} / {\color{red}{8\xspace}}  &  50.0  &  7  &  0  &  \xmark  &  0  &  0  &  \xmark  &  24\\
\hline
\rowcolor[HTML]{ADADAD}
&  total  &  \xspace{}  &  \xspace{} &  {\color{ForestGreen}{\\xspace}} / {\color{red}{x\xspace}}  &  \xspace{}  &  48  &  0  &  2  &  2  &  0  &  3  &  37\\
\hline
\multirow{11}{*}{\rotvertical{commons-lang}}
&  bff7521  &  8/26/18  &  4119 &  {\color{ForestGreen}{2\xspace}} / {\color{red}{8\xspace}}  &  100.0  &  6  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  b1deb44  &  8/26/18  &  4119 &  {\color{ForestGreen}{36\xspace}} / {\color{red}{36\xspace}}  &  100.0  &  4  &  0  &  \xmark  &  0  &  0  &  \xmark  &  27\\
&  f013141  &  8/24/18  &  4119 &  {\color{ForestGreen}{36\xspace}} / {\color{red}{36\xspace}}  &  100.0  &  4  &  0  &  \xmark  &  0  &  0  &  \xmark  &  27\\
&  b31877a  &  8/14/18  &  4116 &  {\color{ForestGreen}{325\xspace}} / {\color{red}{2\xspace}}  &  72.22  &  25  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  a36c903  &  7/27/18  &  4105 &  {\color{ForestGreen}{4\xspace}} / {\color{red}{3\xspace}}  &  100.0  &  50  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  f56931c  &  7/2/18  &  4105 &  {\color{ForestGreen}{30\xspace}} / {\color{red}{4\xspace}}  &  90.0  &  41  &  0  &  \xmark  &  2  &  0  &  \xmark  &  0\\
&  77febcf  &  6/20/18  &  4103 &  {\color{ForestGreen}{27\xspace}} / {\color{red}{29\xspace}}  &  83.33  &  104  &  0  &  \xmark  &  1  &  0  &  \xmark  &  0\\
&  214cc7f  &  6/20/18  &  4103 &  {\color{ForestGreen}{12\xspace}} / {\color{red}{12\xspace}}  &  66.67  &  45  &  0  &  \xmark  &  1  &  0  &  \xmark  &  0\\
&  152e5d4  &  4/19/18  &  4103 &  {\color{ForestGreen}{94\xspace}} / {\color{red}{0\xspace}}  &  88.89  &  4  &  0  &  \xmark  &  0  &  0  &  \xmark  &  4\\
&  81ee0d0  &  5/22/18  &  4101 &  {\color{ForestGreen}{13\xspace}} / {\color{red}{9\xspace}}  &  75.0  &  15  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
\hline
\rowcolor[HTML]{ADADAD}
&  total  &  \xspace{}  &  \xspace{} &  {\color{ForestGreen}{\\xspace}} / {\color{red}{x\xspace}}  &  \xspace{}  &  298  &  0  &  0  &  8  &  0  &  0  &  60\\
\hline
\multirow{11}{*}{\rotvertical{gson}}
&  d8d8ccb  &  7/30/18  &  1050 &  {\color{ForestGreen}{11\xspace}} / {\color{red}{7\xspace}}  &  50.0  &  3  &  0  &  \xmark  &  0  &  0  &  \xmark  &  18\\
&  c1e7e2d  &  7/20/18  &  1050 &  {\color{ForestGreen}{30\xspace}} / {\color{red}{9\xspace}}  &  66.67  &  13  &  0  &  \xmark  &  0  &  0  &  \xmark  &  29\\
&  b1fb9ca  &  9/22/17  &  1035 &  {\color{ForestGreen}{23\xspace}} / {\color{red}{0\xspace}}  &  100.0  &  166  &  0  &  \xmark  &  0  &  0  &  \xmark  &  10\\
&  7a9fd59  &  9/18/17  &  1033 &  {\color{ForestGreen}{21\xspace}} / {\color{red}{2\xspace}}  &  83.33  &  14  &  0  &  \xmark  &  0  &  0  &  \xmark  &  13\\
&  03a72e7  &  8/1/17  &  1031 &  {\color{ForestGreen}{43\xspace}} / {\color{red}{11\xspace}}  &  90.0  &  371  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  ada597e  &  5/31/17  &  1029 &  {\color{ForestGreen}{28\xspace}} / {\color{red}{3\xspace}}  &  100.0  &  5  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  a300148  &  5/31/17  &  1027 &  {\color{ForestGreen}{103\xspace}} / {\color{red}{2\xspace}}  &  100.0  &  664  &  0  &  \xmark  &  0  &  0  &  \xmark  &  9\\
&  9a24219  &  4/19/17  &  1019 &  {\color{ForestGreen}{13\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  36  &  0  &  \xmark  &  1  &  0  &  \xmark  &  125\\
&  9e6f2ba  &  2/16/17  &  1018 &  {\color{ForestGreen}{56\xspace}} / {\color{red}{2\xspace}}  &  100.0  &  9  &  0  &  \xmark  &  0  &  0  &  \xmark  &  1\\
&  44cad04  &  11/26/16  &  1015 &  {\color{ForestGreen}{6\xspace}} / {\color{red}{0\xspace}}  &  100.0  &  2  &  0  &  \xmark  &  0  &  115  &  \cmark  &  2\\
\hline
\rowcolor[HTML]{ADADAD}
&  total  &  \xspace{}  &  \xspace{} &  {\color{ForestGreen}{\\xspace}} / {\color{red}{x\xspace}}  &  \xspace{}  &  1283  &  0  &  0  &  2  &  0  &  1  &  210\\
\hline
\multirow{11}{*}{\rotvertical{jsoup}}
&  26adfcb  &  5/11/18  &  669 &  {\color{ForestGreen}{105\xspace}} / {\color{red}{10\xspace}}  &  75.0  &  26  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  426ffe7  &  5/11/18  &  668 &  {\color{ForestGreen}{27\xspace}} / {\color{red}{46\xspace}}  &  47.06  &  27  &  1  &  \cmark  &  0  &  0  &  \xmark  &  0\\
&  1933e97  &  5/11/18  &  667 &  {\color{ForestGreen}{18\xspace}} / {\color{red}{5\xspace}}  &  50.0  &  24  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  4d10472  &  5/11/18  &  666 &  {\color{ForestGreen}{3\xspace}} / {\color{red}{6\xspace}}  &  60.0  &  5  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  c8c0569  &  5/9/18  &  666 &  {\color{ForestGreen}{89\xspace}} / {\color{red}{62\xspace}}  &  77.97  &  437  &  0  &  \xmark  &  11  &  0  &  \xmark  &  0\\
&  1649122  &  5/6/18  &  666 &  {\color{ForestGreen}{38\xspace}} / {\color{red}{24\xspace}}  &  96.0  &  475  &  1  &  \cmark  &  12  &  0  &  \xmark  &  0\\
&  ae99d7e  &  5/6/18  &  666 &  {\color{ForestGreen}{40\xspace}} / {\color{red}{23\xspace}}  &  85.71  &  482  &  1  &  \cmark  &  13  &  0  &  \xmark  &  0\\
&  eec4cf3  &  5/5/18  &  666 &  {\color{ForestGreen}{8\xspace}} / {\color{red}{1\xspace}}  &  85.71  &  23  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  59f1077  &  5/4/18  &  668 &  {\color{ForestGreen}{64\xspace}} / {\color{red}{19\xspace}}  &  50.0  &  2  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  20ec85e  &  5/2/18  &  668 &  {\color{ForestGreen}{69\xspace}} / {\color{red}{0\xspace}}  &  80.0  &  52  &  0  &  \xmark  &  1  &  0  &  \xmark  &  0\\
\hline
\rowcolor[HTML]{ADADAD}
&  total  &  \xspace{}  &  \xspace{} &  {\color{ForestGreen}{\\xspace}} / {\color{red}{x\xspace}}  &  \xspace{}  &  1553  &  0  &  3  &  40  &  0  &  0  &  0\\
\hline
\multirow{11}{*}{\rotvertical{pdfbox}}
&  4b282a2  &  9/27/18  &  1313 &  {\color{ForestGreen}{1\xspace}} / {\color{red}{34\xspace}}  &  7.14  &  3  &  0  &  \xmark  &  1  &  0  &  \xmark  &  0\\
&  18f2289  &  9/27/18  &  1313 &  {\color{ForestGreen}{9\xspace}} / {\color{red}{3\xspace}}  &  66.67  &  8  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  f6a2c27  &  9/24/18  &  1313 &  {\color{ForestGreen}{2\xspace}} / {\color{red}{2\xspace}}  &  0.0  &  1  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  b09eae6  &  9/21/18  &  1313 &  {\color{ForestGreen}{17\xspace}} / {\color{red}{10\xspace}}  &  50.0  &  3  &  0  &  \xmark  &  1  &  0  &  \xmark  &  0\\
&  241d248  &  9/21/18  &  1313 &  {\color{ForestGreen}{27\xspace}} / {\color{red}{1\xspace}}  &  75.0  &  4  &  0  &  \xmark  &  3  &  0  &  \xmark  &  517\\
&  a6b3b6c  &  9/19/18  &  1313 &  {\color{ForestGreen}{21\xspace}} / {\color{red}{16\xspace}}  &  100.0  &  12  &  0  &  \xmark  &  11  &  0  &  \xmark  &  0\\
&  f83bcc1  &  9/18/18  &  1313 &  {\color{ForestGreen}{5\xspace}} / {\color{red}{2\xspace}}  &  100.0  &  32  &  0  &  \xmark  &  52  &  0  &  \xmark  &  75\\
&  ed24b8c  &  9/11/18  &  1312 &  {\color{ForestGreen}{1\xspace}} / {\color{red}{8\xspace}}  &  40.0  &  13  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  1dba19c  &  9/11/18  &  1312 &  {\color{ForestGreen}{23\xspace}} / {\color{red}{2\xspace}}  &  28.57  &  1  &  0  &  \xmark  &  0  &  0  &  \xmark  &  1\\
&  434e585  &  9/7/18  &  1312 &  {\color{ForestGreen}{57\xspace}} / {\color{red}{50\xspace}}  &  55.0  &  1  &  0  &  \xmark  &  0  &  0  &  \xmark  &  1\\
\hline
\rowcolor[HTML]{ADADAD}
&  total  &  \xspace{}  &  \xspace{} &  {\color{ForestGreen}{\\xspace}} / {\color{red}{x\xspace}}  &  \xspace{}  &  78  &  0  &  0  &  71  &  0  &  0  &  595\\
\hline
\multirow{11}{*}{\rotvertical{xwiki-commons}}
&  ffc3997  &  7/27/18  &  1081 &  {\color{ForestGreen}{125\xspace}} / {\color{red}{18\xspace}}  &  68.75  &  1  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  ced2635  &  8/13/18  &  1081 &  {\color{ForestGreen}{21\xspace}} / {\color{red}{14\xspace}}  &  50.0  &  5  &  0  &  \xmark  &  1  &  0  &  \xmark  &  72\\
&  10841b1  &  8/1/18  &  1061 &  {\color{ForestGreen}{107\xspace}} / {\color{red}{19\xspace}}  &  42.86  &  51  &  0  &  \xmark  &  12  &  0  &  \xmark  &  0\\
&  848c984  &  7/6/18  &  1074 &  {\color{ForestGreen}{154\xspace}} / {\color{red}{111\xspace}}  &  13.33  &  1  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  adfefec  &  6/27/18  &  1073 &  {\color{ForestGreen}{17\xspace}} / {\color{red}{14\xspace}}  &  66.67  &  22  &  0  &  \xmark  &  0  &  0  &  \xmark  &  4\\
&  d3101ae  &  1/18/18  &  1062 &  {\color{ForestGreen}{71\xspace}} / {\color{red}{9\xspace}}  &  60.0  &  4  &  1  &  \cmark  &  0  &  0  &  \xmark  &  0\\
&  a0e8b77  &  1/18/18  &  1062 &  {\color{ForestGreen}{51\xspace}} / {\color{red}{8\xspace}}  &  85.71  &  4  &  1  &  \cmark  &  0  &  0  &  \xmark  &  0\\
&  78ff099  &  12/19/17  &  1061 &  {\color{ForestGreen}{16\xspace}} / {\color{red}{0\xspace}}  &  85.71  &  2  &  0  &  \xmark  &  0  &  0  &  \xmark  &  1\\
&  1b79714  &  11/13/17  &  1060 &  {\color{ForestGreen}{20\xspace}} / {\color{red}{5\xspace}}  &  100.0  &  22  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
&  6dc9059  &  10/31/17  &  1060 &  {\color{ForestGreen}{4\xspace}} / {\color{red}{14\xspace}}  &  62.5  &  22  &  0  &  \xmark  &  0  &  0  &  \xmark  &  0\\
\hline
\rowcolor[HTML]{ADADAD}
&  total  &  \xspace{}  &  \xspace{} &  {\color{ForestGreen}{\\xspace}} / {\color{red}{x\xspace}}  &  \xspace{}  &  134  &  0  &  2  &  15  &  0  &  0  &  78\\
\hline


==> old-stuff/table-content.tex <==
\multirow{10}{*}{\rotvertical{javapoet}}
&\href{https://github.com/square/javapoet/pull/618}{618}&87&8297&$\beta$&\cellcolor[HTML]{FFFE65}80	&	\cellcolor[HTML]{009901}23	&	6m&0	&	0	&	1m&\cellcolor[HTML]{FFFE65}22498	&	\cellcolor[HTML]{009901}2879	&	1205m\\
&\href{https://github.com/square/javapoet/pull/608}{608}&15&8277&$\beta$&0	&	0	&	2s&\cellcolor[HTML]{FFFE65}38	&	0	&	29s&0	&	0	&	10m\\
&\href{https://github.com/square/javapoet/pull/605}{605}&1&8277&$\beta$&\cellcolor[HTML]{FFFE65}1	&	\cellcolor[HTML]{009901}1	&	8s&0	&	0	&	1s&0	&	0	&5s\\
&\href{https://github.com/square/javapoet/pull/567}{567}&43&8042&$\beta$&\cellcolor[HTML]{FFFE65}15	&	0	&	22s&0	&	0	&	23s&\cellcolor[HTML]{FFFE65}5104	&	0&	50m\\
&\href{https://github.com/square/javapoet/pull/562}{562}&27&8032&$\beta$&\cellcolor[HTML]{FFFE65}22	&	\cellcolor[HTML]{009901}6	&	2m&0	&	0	&	32s&\cellcolor[HTML]{FFFE65}5185	&	\cellcolor[HTML]{009901}480	&	331m\\
&\href{https://github.com/square/javapoet/pull/550}{550}&11&7896&$\beta$&\cellcolor[HTML]{FFFE65}6	&	0	&	15s&0	&	0	&	11s&\cellcolor[HTML]{FFFE65}665	&	0	&13m\\
&\href{https://github.com/square/javapoet/pull/529}{529}&29&7874&$\alpha$&\cellcolor[HTML]{FFFE65}9	&	0	&	8s&0	&	0	&	11s&\cellcolor[HTML]{FFFE65}4355	&	0&	34m\\
&\href{https://github.com/square/javapoet/pull/526}{526}&25&7536&$\beta$&\cellcolor[HTML]{FFFE65}21	&	\cellcolor[HTML]{009901}6	&	2m&0	&	0	&	30s&\cellcolor[HTML]{FFFE65}4873	&	\cellcolor[HTML]{009901}481	&	149m\\
&\href{https://github.com/square/javapoet/pull/524}{524}&102&7523&$\beta$&\cellcolor[HTML]{FFFE65}77	&	0	&	1m&\cellcolor[HTML]{FFFE65}2	&	0	&	1m&&&\\
&\href{https://github.com/square/javapoet/pull/469}{469}&98&7377&$\beta$&\cellcolor[HTML]{FFFE65}75	&	0	&	1m&0	&	0	&	1m&&&\\
\hline
\multirow{10}{*}{\rotvertical{jsoup}}
&\href{https://github.com/jhy/jsoup/pull/1046}{1046}&7&19318&$\beta$&\cellcolor[HTML]{FFFE65}6	&	0	&	8s&\cellcolor[HTML]{FFFE65}2	&	0	&	5m&\cellcolor[HTML]{FFFE65}1297	&	\cellcolor[HTML]{009901}3	&	37m\\
&\href{https://github.com/jhy/jsoup/pull/1038}{1038}&21&19243&$\alpha$&\cellcolor[HTML]{FFFE65}5	&	0	&	112m&0	&	0	&	9s&\cellcolor[HTML]{FFFE65}1156	&	0	&1124m\\
&\href{https://github.com/jhy/jsoup/pull/988}{988}&2&19140&$\beta$&\cellcolor[HTML]{FFFE65}2	&	\cellcolor[HTML]{009901}2	&	2s&0	&	0	&	1s&\cellcolor[HTML]{FFFE65}2&	0	&	10s\\
&\href{https://github.com/jhy/jsoup/pull/942}{942}&114&17426&$\beta$&\cellcolor[HTML]{FFFE65}111	&	\cellcolor[HTML]{009901}2	&	1m&\cellcolor[HTML]{FFFE65}8	&	0	&	1m&&&\\
&\href{https://github.com/jhy/jsoup/pull/931}{931}&2&17426&$\alpha$&\cellcolor[HTML]{FFFE65}2	&	0	&	2s&\cellcolor[HTML]{FFFE65}5	&	0	&	3s&\cellcolor[HTML]{FFFE65}313	&	0	&	40s\\
&\href{https://github.com/jhy/jsoup/pull/918}{918}&4&17454&$\beta$&\cellcolor[HTML]{FFFE65}1	&	\cellcolor[HTML]{009901}1	&	16s&0	&	0	&	3s&\cellcolor[HTML]{FFFE65}945	&	0	&	2m\\
&\href{https://github.com/jhy/jsoup/pull/903}{903}&3&16784&$\beta$&\cellcolor[HTML]{FFFE65}3	&	\cellcolor[HTML]{009901}2	&	23s&\cellcolor[HTML]{FFFE65}4	&	0	&	6s&\cellcolor[HTML]{FFFE65}684	&	0	&	6m\\
&\href{https://github.com/jhy/jsoup/pull/901}{901}&108&16784&$\beta$&\cellcolor[HTML]{FFFE65}105	&	\cellcolor[HTML]{009901}90	&	24m&\cellcolor[HTML]{FFFE65}6	&	0	&	1m&\cellcolor[HTML]{FFFE65}7167	&	\cellcolor[HTML]{009901}64	&	101m\\
&\href{https://github.com/jhy/jsoup/pull/881}{881}&19&16464&$\alpha$&\cellcolor[HTML]{FFFE65}9	&	\cellcolor[HTML]{009901}5	&	88m&0	&	0	&	8s&\cellcolor[HTML]{FFFE65}1315	&	0	&	1099m\\
&\href{https://github.com/jhy/jsoup/pull/835}{835}&11&16464&$\beta$&\cellcolor[HTML]{FFFE65}8	&	\cellcolor[HTML]{009901}3	&	25s&0	&	0	&	4s&\cellcolor[HTML]{FFFE65}1218	&	0	&	6m\\
\hline
\multirow{10}{*}{\rotvertical{mybatis-3}}
&\href{https://github.com/mybatis/mybatis-3/pull/1250}{1250}&1&56696&$\beta$&\cellcolor[HTML]{FFFE65}1	&	0	&	7s&0	&	0	&	2s&\cellcolor[HTML]{FFFE65}39	&	0	&44s\\
&\href{https://github.com/mybatis/mybatis-3/pull/1149}{1149}&9&56401&$\alpha$&\cellcolor[HTML]{FFFE65}8	&	\cellcolor[HTML]{009901}2	&	6s&\cellcolor[HTML]{FFFE65}1542	&	0	&	2m&\cellcolor[HTML]{FFFE65}1525	&	\cellcolor[HTML]{009901}25	&	3m\\
&\href{https://github.com/mybatis/mybatis-3/pull/1110}{1110}&18&56191&$\alpha$&\cellcolor[HTML]{FFFE65}15	&	\cellcolor[HTML]{009901}6	&	40s&0	&	0	&	37s&\cellcolor[HTML]{FFFE65}3170	&	\cellcolor[HTML]{009901}1	&	76m\\
&\href{https://github.com/mybatis/mybatis-3/pull/1084}{1084}&5&55962&$\beta$&\cellcolor[HTML]{FFFE65}5	&	0	&	17s&0	&	0	&	8s&\cellcolor[HTML]{FFFE65}1215	&	0	&106m\\
&\href{https://github.com/mybatis/mybatis-3/pull/1073}{1073}&1&55825&$\beta$&\cellcolor[HTML]{FFFE65}1	&	\cellcolor[HTML]{009901}1	&	7s&0	&	0	&	2s&\cellcolor[HTML]{FFFE65}13	&	\cellcolor[HTML]{009901}13	&	13s\\
&\href{https://github.com/mybatis/mybatis-3/pull/1070}{1070}&8&55825&$\beta$&\cellcolor[HTML]{FFFE65}7	&	0	&	7s&\cellcolor[HTML]{FFFE65}7	&	0	&	14s&\cellcolor[HTML]{FFFE65}791	&	\cellcolor[HTML]{009901}4	&	3m\\
&\href{https://github.com/mybatis/mybatis-3/pull/976}{976}&7&53995&$\beta$&\cellcolor[HTML]{FFFE65}2	&	0	&	4s&0	&	0	&	4s&0	&	0	&	7s\\
&\href{https://github.com/mybatis/mybatis-3/pull/947}{947}&6&53918&$\beta$&\cellcolor[HTML]{FFFE65}2	&	0	&	4s&0	&	0	&	4s&0	&	0	&	6s\\
&\href{https://github.com/mybatis/mybatis-3/pull/926}{926}&21&53751&$\beta$&\cellcolor[HTML]{FFFE65}21	&	\cellcolor[HTML]{009901}4	&	7s&0	&	0	&	8s&\cellcolor[HTML]{FFFE65}1434	&	0	&	5m\\
&\href{https://github.com/mybatis/mybatis-3/pull/895}{895}&2&52937&$\beta$&\cellcolor[HTML]{FFFE65}2	&	0	&	14s&0	&	0	&	6s&\cellcolor[HTML]{FFFE65}109	&	0	&265m\\
\hline
\multirow{6}{*}{\rotvertical{protostuff}}
&\href{https://github.com/protostuff/protostuff/pull/201}{201}&1&80306&$\alpha$&0	&	0	&	4s&0	&	0	&	2s&\cellcolor[HTML]{FFFE65}2	&	0	&	10s\\
&\href{https://github.com/protostuff/protostuff/pull/185}{185}&1&79442&$\alpha$&0	&	0	&	3s&0	&	0	&	1s&\cellcolor[HTML]{FFFE65}1	&	0	&	5s\\
&\href{https://github.com/protostuff/protostuff/pull/184}{184}&3&79526&$\beta$&\cellcolor[HTML]{FFFE65}3	&	0	&	5s&0	&	0	&	1s&\cellcolor[HTML]{FFFE65}1322	&	0&	3m\\
&\href{https://github.com/protostuff/protostuff/pull/182}{182}&2&79147&$\alpha$&0	&	0	&	8s&0	&	0	&	3s&\cellcolor[HTML]{FFFE65}3	&	0	&	15s\\
&\href{https://github.com/protostuff/protostuff/pull/180}{180}&2&78417&$\beta$&0	&	0	&	7s&0	&	0	&	3s&\cellcolor[HTML]{FFFE65}3	&	0	&	14s\\
&\href{https://github.com/protostuff/protostuff/pull/119}{119}&4&78890&$\beta$&\cellcolor[HTML]{FFFE65}2	&	\cellcolor[HTML]{009901}1	&	2m&0	&	0	&	2s&\cellcolor[HTML]{FFFE65}2	&	0	&	13s\\


==> old-stuff/table.tex <==
\begin{table*}
\centering
\small
\def\arraystretch{1}%  1 is the default, change whatever you need
\setlength\tabcolsep{6pt} % default value: 6pt
\begin{tabular}{l|cccc
|ccc
|ccc
|ccc}
&   &	&	&   &
\multicolumn{3}{c}{\aampl}&
\multicolumn{3}{c}{aaa}&
\multicolumn{3}{c}{\iampl}\\
\hline
\rotvertical{Project} &
ID &\rotvertical{\# Test Methods} & \#LOC &\rotvertical{Sanity} & 
\rotvertical{\# Amplified} & \rotvertical{\# Success} & \rotvertical{Time} &
\rotvertical{\# Amplified} & \rotvertical{\# Success} & \rotvertical{Time} &
\rotvertical{\# Amplified} & \rotvertical{\# Success} & \rotvertical{Time}\\ 
\hline
\input{table-content}
\end{tabular}
\caption{\TODO{caption}}
\label{tab:overall-result}
\end{table*}

==> table_content.tex <==
&
id&
date&
\#Test&
\begin{tabular}{c}\#Modified\\Tests\end{tabular}&
{\color{ForestGreen}{+\xspace}} / {\color{red}{-\xspace}}&
Cov&
\begin{tabular}{c}\#Selected\\Tests\end{tabular}&
\begin{tabular}{c}\#\aampl\\Tests\end{tabular}&
Time&
\begin{tabular}{c}\#\sbampl\\Tests\end{tabular}&
Time\\\\
\midrule
\multirow{11}{*}{\rotvertical{commons-io}}
&  c6b8a38  &  6/12/18 &  1348  &  2  &  {\color{ForestGreen}{104\xspace}} / {\color{red}{3\xspace}}  &  100.0  &  3  &  0  &  10.0s  &  0  &  98.0s\\
&  2736b6f  &  12/21/17 &  1343  &  2  &  {\color{ForestGreen}{164\xspace}} / {\color{red}{1\xspace}}  &  1.79  &  8  &  0  &  19.0s  &  \cmark(12)  &  76.3m\\
&  a4705cc  &  4/29/18 &  1328  &  1  &  {\color{ForestGreen}{37\xspace}} / {\color{red}{0\xspace}}  &  100.0  &  2  &  0  &  10.0s  &  0  &  38.1m\\
&  f00d97a  &  5/2/17 &  1316  &  10  &  {\color{ForestGreen}{244\xspace}} / {\color{red}{25\xspace}}  &  100.0  &  2  &  \cmark(1)  &  10.0s  &  \cmark(39)  &  27.0s\\
&  3378280  &  4/25/17 &  1309  &  2  &  {\color{ForestGreen}{5\xspace}} / {\color{red}{5\xspace}}  &  100.0  &  1  &  \cmark(1)  &  9.0s  &  \cmark(11)  &  24.0s\\
&  703228a  &  12/2/16 &  1309  &  1  &  {\color{ForestGreen}{6\xspace}} / {\color{red}{0\xspace}}  &  50.0  &  8  &  0  &  19.0s  &  0  &  71.0m\\
&  a7bd568  &  9/24/16 &  1163  &  1  &  {\color{ForestGreen}{91\xspace}} / {\color{red}{83\xspace}}  &  50.0  &  8  &  0  &  20.0s  &  0  &  65.2m\\
&  81210eb  &  6/2/16 &  1160  &  1  &  {\color{ForestGreen}{10\xspace}} / {\color{red}{2\xspace}}  &  100.0  &  1  &  0  &  8.0s  &  \cmark(8)  &  23.0s\\
&  57f493a  &  11/19/15 &  1153  &  1  &  {\color{ForestGreen}{15\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  8  &  0  &  7.0s  &  0  &  54.0s\\
&  5d072ef  &  9/10/15 &  1125  &  12  &  {\color{ForestGreen}{74\xspace}} / {\color{red}{34\xspace}}  &  68.42  &  25  &  \cmark(6)  &  29.0s  &  \cmark(1538)  &  2.2h\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  66  &  8  &  2.4m  &  1608  &  6.5h\\
\midrule
&  average  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  6.60  &  0.80  &  14.5s  &  160.80  &  38.8m\\
\midrule
\multirow{11}{*}{\rotvertical{commons-lang}}
&  f56931c  &  7/2/18 &  4105  &  1  &  {\color{ForestGreen}{30\xspace}} / {\color{red}{4\xspace}}  &  25.0  &  42  &  0  &  2.4m  &  0  &  8.5m\\
&  87937b2  &  5/22/18 &  4101  &  1  &  {\color{ForestGreen}{114\xspace}} / {\color{red}{0\xspace}}  &  77.78  &  16  &  0  &  35.0s  &  0  &  18.1m\\
&  09ef69c  &  5/18/18 &  4100  &  1  &  {\color{ForestGreen}{10\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  4  &  0  &  16.0s  &  0  &  98.8m\\
&  3fadfdd  &  5/10/18 &  4089  &  1  &  {\color{ForestGreen}{7\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  9  &  0  &  17.0s  &  \cmark(4)  &  17.2m\\
&  e7d16c2  &  5/9/18 &  4088  &  1  &  {\color{ForestGreen}{13\xspace}} / {\color{red}{1\xspace}}  &  33.33  &  7  &  0  &  16.0s  &  \cmark(2)  &  15.1m\\
&  50ce8c4  &  3/8/18 &  4084  &  4  &  {\color{ForestGreen}{40\xspace}} / {\color{red}{1\xspace}}  &  90.91  &  2  &  \cmark(1)  &  28.0s  &  \cmark(135)  &  2.0m\\
&  2e9f3a8  &  2/11/18 &  4084  &  2  &  {\color{ForestGreen}{79\xspace}} / {\color{red}{4\xspace}}  &  30.0  &  47  &  0  &  79.0s  &  0  &  66.5m\\
&  c8e61af  &  2/10/18 &  4082  &  1  &  {\color{ForestGreen}{8\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  10  &  0  &  17.0s  &  0  &  16.0s\\
&  d8ec011  &  11/12/17 &  4074  &  1  &  {\color{ForestGreen}{11\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  5  &  0  &  31.0s  &  0  &  2.3m\\
&  7d061e3  &  11/22/17 &  4073  &  1  &  {\color{ForestGreen}{16\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  8  &  0  &  17.0s  &  0  &  11.4m\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  150  &  1  &  6.7m  &  141  &  4.0h\\
\midrule
&  average  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  15.00  &  0.10  &  40.5s  &  14.10  &  24.0m\\
\midrule
\multirow{11}{*}{\rotvertical{gson}}
&  b1fb9ca  &  9/22/17 &  1035  &  1  &  {\color{ForestGreen}{23\xspace}} / {\color{red}{0\xspace}}  &  50.0  &  166  &  0  &  4.2m  &  0  &  92.5m\\
&  7a9fd59  &  9/18/17 &  1033  &  2  &  {\color{ForestGreen}{21\xspace}} / {\color{red}{2\xspace}}  &  83.33  &  14  &  0  &  15.0s  &  \cmark(108)  &  2.1m\\
&  03a72e7  &  8/1/17 &  1031  &  2  &  {\color{ForestGreen}{43\xspace}} / {\color{red}{11\xspace}}  &  68.75  &  371  &  0  &  7.7m  &  0  &  3.2h\\
&  74e3711  &  6/20/17 &  1029  &  1  &  {\color{ForestGreen}{68\xspace}} / {\color{red}{5\xspace}}  &  8.0  &  1  &  0  &  4.0s  &  0  &  16.0s\\
&  ada597e  &  5/31/17 &  1029  &  2  &  {\color{ForestGreen}{28\xspace}} / {\color{red}{3\xspace}}  &  100.0  &  5  &  0  &  8.0s  &  0  &  8.7m\\
&  a300148  &  5/31/17 &  1027  &  7  &  {\color{ForestGreen}{103\xspace}} / {\color{red}{2\xspace}}  &  18.18  &  665  &  0  &  9.2m  &  \cmark(6)  &  4.9h\\
&  9a24219  &  4/19/17 &  1019  &  1  &  {\color{ForestGreen}{13\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  36  &  0  &  2.2m  &  0  &  48.9m\\
&  9e6f2ba  &  2/16/17 &  1018  &  2  &  {\color{ForestGreen}{56\xspace}} / {\color{red}{2\xspace}}  &  50.0  &  9  &  0  &  32.0s  &  \cmark(2)  &  8.5m\\
&  44cad04  &  11/26/16 &  1015  &  1  &  {\color{ForestGreen}{6\xspace}} / {\color{red}{0\xspace}}  &  100.0  &  2  &  0  &  15.0s  &  \cmark(37)  &  40.0s\\
&  b2c00a3  &  6/14/16 &  1012  &  4  &  {\color{ForestGreen}{242\xspace}} / {\color{red}{29\xspace}}  &  60.71  &  383  &  0  &  7.9m  &  0  &  3.6h\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  1652  &  0  &  32.4m  &  153  &  14.4h\\
\midrule
&  average  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  165.20  &  0.00  &  3.2m  &  15.30  &  86.5m\\
\midrule
\multirow{11}{*}{\rotvertical{jsoup}}
&  426ffe7  &  5/11/18 &  668  &  4  &  {\color{ForestGreen}{27\xspace}} / {\color{red}{46\xspace}}  &  64.71  &  27  &  \cmark(2)  &  42.0s  &  \cmark(198)  &  33.6m\\
&  a810d2e  &  4/29/18 &  666  &  1  &  {\color{ForestGreen}{27\xspace}} / {\color{red}{1\xspace}}  &  80.0  &  5  &  0  &  10.0s  &  0  &  26.6m\\
&  6be19a6  &  4/29/18 &  664  &  1  &  {\color{ForestGreen}{23\xspace}} / {\color{red}{1\xspace}}  &  50.0  &  50  &  0  &  69.0s  &  0  &  67.7m\\
&  e38dfd4  &  4/28/18 &  659  &  1  &  {\color{ForestGreen}{66\xspace}} / {\color{red}{15\xspace}}  &  90.0  &  18  &  0  &  35.0s  &  0  &  12.5m\\
&  e9feec9  &  4/15/18 &  654  &  1  &  {\color{ForestGreen}{15\xspace}} / {\color{red}{3\xspace}}  &  100.0  &  4  &  0  &  9.0s  &  0  &  95.0s\\
&  0f7e0cc  &  4/14/18 &  653  &  2  &  {\color{ForestGreen}{56\xspace}} / {\color{red}{15\xspace}}  &  84.62  &  330  &  0  &  6.5m  &  \cmark(36)  &  11.8h\\
&  2c4e79b  &  4/14/18 &  650  &  2  &  {\color{ForestGreen}{82\xspace}} / {\color{red}{2\xspace}}  &  50.0  &  44  &  0  &  67.0s  &  0  &  4.7h\\
&  e5210d1  &  12/22/17 &  647  &  1  &  {\color{ForestGreen}{3\xspace}} / {\color{red}{3\xspace}}  &  100.0  &  14  &  0  &  9.0s  &  0  &  4.9m\\
&  df272b7  &  12/22/17 &  647  &  2  &  {\color{ForestGreen}{17\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  13  &  0  &  9.0s  &  0  &  4.6m\\
&  3676b13  &  12/21/17 &  648  &  6  &  {\color{ForestGreen}{104\xspace}} / {\color{red}{12\xspace}}  &  38.46  &  239  &  0  &  6.2m  &  \cmark(52)  &  6.8h\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  744  &  2  &  16.8m  &  286  &  25.8h\\
\midrule
&  average  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  74.40  &  0.20  &  101.0s  &  28.60  &  2.6h\\
\midrule
\multirow{11}{*}{\rotvertical{mustache.java}}
&  a1197f7  &  1/25/18 &  228  &  1  &  {\color{ForestGreen}{43\xspace}} / {\color{red}{57\xspace}}  &  77.78  &  131  &  0  &  11.8m  &  \cmark(204)  &  10.1h\\
&  8877027  &  11/19/17 &  227  &  1  &  {\color{ForestGreen}{22\xspace}} / {\color{red}{2\xspace}}  &  33.33  &  47  &  0  &  7.3m  &  0  &  100.2m\\
&  d8936b4  &  2/1/17 &  219  &  2  &  {\color{ForestGreen}{46\xspace}} / {\color{red}{6\xspace}}  &  60.0  &  168  &  0  &  12.7m  &  0  &  84.2m\\
&  88718bc  &  1/25/17 &  216  &  2  &  {\color{ForestGreen}{29\xspace}} / {\color{red}{1\xspace}}  &  100.0  &  1  &  \cmark(1)  &  7.0s  &  \cmark(149)  &  3.7m\\
&  339161f  &  9/23/16 &  214  &  2  &  {\color{ForestGreen}{32\xspace}} / {\color{red}{10\xspace}}  &  77.78  &  123  &  0  &  8.6m  &  \cmark(1312)  &  5.8h\\
&  774ae7a  &  8/10/16 &  214  &  2  &  {\color{ForestGreen}{17\xspace}} / {\color{red}{2\xspace}}  &  100.0  &  11  &  0  &  66.0s  &  \cmark(124)  &  6.8m\\
&  94847cc  &  7/29/16 &  214  &  2  &  {\color{ForestGreen}{17\xspace}} / {\color{red}{2\xspace}}  &  100.0  &  95  &  0  &  11.5m  &  \cmark(2509)  &  21.4h\\
&  eca08ca  &  7/14/16 &  212  &  4  &  {\color{ForestGreen}{47\xspace}} / {\color{red}{10\xspace}}  &  80.0  &  18  &  0  &  87.0s  &  0  &  41.8m\\
&  6d7225c  &  7/7/16 &  212  &  2  &  {\color{ForestGreen}{42\xspace}} / {\color{red}{4\xspace}}  &  80.0  &  18  &  0  &  87.0s  &  0  &  40.1m\\
&  8ac71b7  &  7/6/16 &  210  &  10  &  {\color{ForestGreen}{167\xspace}} / {\color{red}{31\xspace}}  &  40.0  &  20  &  0  &  2.1m  &  \cmark(124)  &  5.6m\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  632  &  1  &  58.1m  &  4422  &  42.0h\\
\midrule
&  average  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  63.20  &  0.10  &  5.8m  &  442.20  &  4.2h\\
\midrule
\multirow{11}{*}{\rotvertical{xwiki-commons}}
&  ffc3997  &  7/27/18 &  1081  &  0  &  {\color{ForestGreen}{125\xspace}} / {\color{red}{18\xspace}}  &  21.05  &  1  &  0  &  29.0s  &  0  &  18.0s\\
&  ced2635  &  8/13/18 &  1081  &  1  &  {\color{ForestGreen}{21\xspace}} / {\color{red}{14\xspace}}  &  60.0  &  5  &  0  &  93.0s  &  0  &  2.5h\\
&  10841b1  &  8/1/18 &  1061  &  1  &  {\color{ForestGreen}{107\xspace}} / {\color{red}{19\xspace}}  &  30.0  &  51  &  0  &  5.7m  &  0  &  3.4h\\
&  848c984  &  7/6/18 &  1074  &  1  &  {\color{ForestGreen}{154\xspace}} / {\color{red}{111\xspace}}  &  17.65  &  1  &  0  &  28.0s  &  0  &  18.0s\\
&  adfefec  &  6/27/18 &  1073  &  1  &  {\color{ForestGreen}{17\xspace}} / {\color{red}{14\xspace}}  &  40.0  &  22  &  \cmark(1)  &  76.0s  &  \cmark(3)  &  14.9m\\
&  d3101ae  &  1/18/18 &  1062  &  2  &  {\color{ForestGreen}{71\xspace}} / {\color{red}{9\xspace}}  &  20.0  &  4  &  \cmark(1)  &  72.0s  &  \cmark(31)  &  41.4m\\
&  a0e8b77  &  1/18/18 &  1062  &  2  &  {\color{ForestGreen}{51\xspace}} / {\color{red}{8\xspace}}  &  42.86  &  4  &  \cmark(1)  &  72.0s  &  \cmark(60)  &  42.1m\\
&  78ff099  &  12/19/17 &  1061  &  1  &  {\color{ForestGreen}{16\xspace}} / {\color{red}{0\xspace}}  &  33.33  &  2  &  0  &  68.0s  &  \cmark(4)  &  6.6m\\
&  1b79714  &  11/13/17 &  1060  &  1  &  {\color{ForestGreen}{20\xspace}} / {\color{red}{5\xspace}}  &  60.0  &  22  &  0  &  78.0s  &  0  &  17.9m\\
&  6dc9059  &  10/31/17 &  1060  &  1  &  {\color{ForestGreen}{4\xspace}} / {\color{red}{14\xspace}}  &  88.89  &  22  &  0  &  79.0s  &  0  &  20.5m\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  134  &  3  &  15.7m  &  98  &  8.2h\\
\midrule
&  average  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  13.40  &  0.30  &  94.3s  &  9.80  &  49.5m\\
\midrule
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  \xspace{} &  \xspace{}  &  \xspace{}  &  \xspace{}  &  \xspace{}  &  3378  &  9(15)  &  2.2h  &  25(6708)  &  100.9h\\
\bottomrule

==> table_content_iterations.tex <==
&
id&
$it=1$&
Time&
$it=2$&
Time&
$it=3$&
Time\\
\midrule
\multirow{11}{*}{\rotvertical{commons-io}}
&  c6b8a38  &  0 &  25.0s  &  0  &  62.0s  &  0  &  98.0s\\
&  2736b6f  &  \cmark(1) &  26.1m  &  \cmark(2)  &  44.2m  &  \cmark(12)  &  76.3m\\
&  a4705cc  &  0 &  4.1m  &  0  &  21.1m  &  0  &  38.1m\\
&  f00d97a  &  \cmark(7) &  13.0s  &  \cmark(28)  &  19.0s  &  \cmark(39)  &  27.0s\\
&  3378280  &  \cmark(6) &  15.0s  &  \cmark(10)  &  20.0s  &  \cmark(11)  &  24.0s\\
&  703228a  &  0 &  30.3m  &  0  &  55.1m  &  0  &  71.0m\\
&  a7bd568  &  0 &  28.6m  &  0  &  52.0m  &  0  &  65.2m\\
&  81210eb  &  \cmark(2) &  14.0s  &  \cmark(4)  &  18.0s  &  \cmark(8)  &  23.0s\\
&  57f493a  &  0 &  20.0s  &  0  &  32.0s  &  0  &  54.0s\\
&  5d072ef  &  \cmark(461) &  32.2m  &  \cmark(1014)  &  65.5m  &  \cmark(1538)  &  2.2h\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  477 &  2.0h  &  1058  &  4.0h  &  1608  &  6.5h\\
\midrule
&  average  &  47.70 &  12.3m  &  105.80  &  24.0m  &  160.80  &  38.8m\\
\midrule
\multirow{11}{*}{\rotvertical{commons-lang}}
&  f56931c  &  0 &  0.0s  &  0  &  3.7m  &  0  &  8.5m\\
&  87937b2  &  0 &  3.5m  &  0  &  10.5m  &  0  &  18.1m\\
&  09ef69c  &  0 &  97.0s  &  0  &  21.0m  &  0  &  98.8m\\
&  3fadfdd  &  \cmark(1) &  2.0m  &  \cmark(1)  &  9.3m  &  \cmark(4)  &  17.2m\\
&  e7d16c2  &  \cmark(3) &  111.0s  &  \cmark(2)  &  8.4m  &  \cmark(2)  &  15.1m\\
&  50ce8c4  &  \cmark(61) &  38.0s  &  \cmark(97)  &  78.0s  &  \cmark(135)  &  2.0m\\
&  2e9f3a8  &  0 &  11.4m  &  0  &  35.0m  &  0  &  66.5m\\
&  c8e61af  &  0 &  16.0s  &  0  &  16.0s  &  0  &  16.0s\\
&  d8ec011  &  0 &  36.0s  &  0  &  68.0s  &  0  &  2.3m\\
&  7d061e3  &  0 &  79.0s  &  0  &  5.8m  &  0  &  11.4m\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  65 &  23.3m  &  100  &  96.4m  &  141  &  4.0h\\
\midrule
&  average  &  6.50 &  2.3m  &  10.00  &  9.6m  &  14.10  &  24.0m\\
\midrule
\multirow{11}{*}{\rotvertical{gson}}
&  b1fb9ca  &  0 &  14.6m  &  0  &  51.0m  &  0  &  92.5m\\
&  7a9fd59  &  \cmark(7) &  33.0s  &  \cmark(48)  &  73.0s  &  \cmark(108)  &  2.1m\\
&  03a72e7  &  0 &  30.2m  &  0  &  102.3m  &  0  &  3.2h\\
&  74e3711  &  0 &  6.0s  &  0  &  11.0s  &  0  &  16.0s\\
&  ada597e  &  0 &  61.0s  &  0  &  4.9m  &  0  &  8.7m\\
&  a300148  &  0 &  45.2m  &  \cmark(4)  &  2.6h  &  \cmark(6)  &  4.9h\\
&  9a24219  &  0 &  10.8m  &  0  &  28.4m  &  0  &  48.9m\\
&  9e6f2ba  &  0 &  79.0s  &  0  &  4.5m  &  \cmark(2)  &  8.5m\\
&  44cad04  &  \cmark(4) &  21.0s  &  \cmark(21)  &  30.0s  &  \cmark(37)  &  40.0s\\
&  b2c00a3  &  0 &  31.5m  &  0  &  111.8m  &  0  &  3.6h\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  11 &  2.3h  &  73  &  7.7h  &  153  &  14.4h\\
\midrule
&  average  &  1.10 &  13.6m  &  7.30  &  46.0m  &  15.30  &  86.5m\\
\midrule
\multirow{11}{*}{\rotvertical{jsoup}}
&  426ffe7  &  \cmark(126) &  5.4m  &  \cmark(172)  &  19.2m  &  \cmark(198)  &  33.6m\\
&  a810d2e  &  0 &  90.0s  &  0  &  13.9m  &  0  &  26.6m\\
&  6be19a6  &  0 &  8.1m  &  0  &  39.7m  &  0  &  67.7m\\
&  e38dfd4  &  0 &  117.0s  &  0  &  6.3m  &  0  &  12.5m\\
&  e9feec9  &  0 &  20.0s  &  0  &  50.0s  &  0  &  95.0s\\
&  0f7e0cc  &  \cmark(1) &  2.4h  &  \cmark(7)  &  6.8h  &  \cmark(36)  &  11.8h\\
&  2c4e79b  &  0 &  7.1m  &  0  &  34.1m  &  0  &  4.7h\\
&  e5210d1  &  0 &  45.0s  &  0  &  2.3m  &  0  &  4.9m\\
&  df272b7  &  0 &  43.0s  &  0  &  2.2m  &  0  &  4.6m\\
&  3676b13  &  \cmark(6) &  21.4m  &  \cmark(35)  &  2.9h  &  \cmark(52)  &  6.8h\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  133 &  3.2h  &  214  &  11.6h  &  286  &  25.8h\\
\midrule
&  average  &  13.30 &  19.4m  &  21.40  &  69.8m  &  28.60  &  2.6h\\
\midrule
\multirow{11}{*}{\rotvertical{mustache.java}}
&  a1197f7  &  \cmark(28) &  5.9h  &  \cmark(124)  &  8.4h  &  \cmark(204)  &  10.1h\\
&  8877027  &  0 &  30.5m  &  0  &  58.4m  &  0  &  100.2m\\
&  d8936b4  &  0 &  3.2m  &  0  &  4.8m  &  0  &  84.2m\\
&  88718bc  &  \cmark(13) &  78.0s  &  \cmark(85)  &  2.5m  &  \cmark(149)  &  3.7m\\
&  339161f  &  \cmark(143) &  115.9m  &  \cmark(699)  &  4.1h  &  \cmark(1312)  &  5.8h\\
&  774ae7a  &  \cmark(18) &  2.7m  &  \cmark(65)  &  4.7m  &  \cmark(124)  &  6.8m\\
&  94847cc  &  \cmark(122) &  5.3h  &  \cmark(580)  &  10.4h  &  \cmark(2509)  &  21.4h\\
&  eca08ca  &  0 &  8.1m  &  0  &  24.3m  &  0  &  41.8m\\
&  6d7225c  &  0 &  7.9m  &  0  &  26.8m  &  0  &  40.1m\\
&  8ac71b7  &  \cmark(2) &  2.7m  &  \cmark(48)  &  3.8m  &  \cmark(124)  &  5.6m\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  326 &  14.0h  &  1601  &  25.0h  &  4422  &  42.0h\\
\midrule
&  average  &  32.60 &  84.3m  &  160.10  &  2.5h  &  442.20  &  4.2h\\
\midrule
\multirow{11}{*}{\rotvertical{xwiki-commons}}
&  ffc3997  &  0 &  19.0s  &  0  &  18.0s  &  0  &  18.0s\\
&  ced2635  &  0 &  8.0m  &  0  &  31.8m  &  0  &  2.5h\\
&  10841b1  &  0 &  56.2m  &  0  &  2.9h  &  0  &  3.4h\\
&  848c984  &  0 &  18.0s  &  0  &  17.0s  &  0  &  18.0s\\
&  adfefec  &  \cmark(22) &  3.5m  &  \cmark(57)  &  9.9m  &  \cmark(3)  &  14.9m\\
&  d3101ae  &  \cmark(9) &  11.6m  &  \cmark(12)  &  28.2m  &  \cmark(31)  &  41.4m\\
&  a0e8b77  &  \cmark(10) &  12.0m  &  \cmark(17)  &  28.2m  &  \cmark(60)  &  42.1m\\
&  78ff099  &  \cmark(4) &  2.6m  &  \cmark(4)  &  4.6m  &  \cmark(4)  &  6.6m\\
&  1b79714  &  0 &  4.0m  &  0  &  10.7m  &  0  &  17.9m\\
&  6dc9059  &  0 &  4.0m  &  0  &  10.8m  &  0  &  20.5m\\
\midrule
\rowcolor[HTML]{EFEFEF}
&  total  &  45 &  102.8m  &  90  &  4.9h  &  98  &  8.2h\\
\midrule
&  average  &  4.50 &  10.3m  &  9.00  &  29.7m  &  9.80  &  49.5m\\
\midrule
\midrule
&  total  &  23(1057) &  23.7h  &  24(3136)  &  54.9h  &  25(6708)  &  100.9h\\
\bottomrule

==> table_content_seeds.tex <==
&id&ref&0&1&2&3&4&5&6&7&8&9\\
\hline
\multirow{11}{*}{\rotvertical{commons-io}}
 & c6b8a38 & - & - & - & - & - & - & - & - & - & - & -\\
 & 2736b6f & 1 & 1 & 1 & - & 2 & 1 & 1 & 2 & 1 & - & -\\
 & a4705cc & - & - & - & - & - & - & - & - & - & - & -\\
 & f00d97a & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7\\
 & 3378280 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6\\
 & 703228a & - & - & - & - & - & - & 2 & - & 1 & - & -\\
 & a7bd568 & - & - & - & - & - & - & 2 & - & 1 & - & -\\
 & 81210eb & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2\\
 & 57f493a & - & - & - & - & - & - & - & - & - & - & -\\
 & 5d072ef & 461 & 464 & 462 & 463 & 463 & 461 & 462 & 465 & 460 & 463 & 462\\
\hline
\multirow{11}{*}{\rotvertical{commons-lang}}
 & f56931c & - & - & - & - & - & 1 & - & 1 & 1 & 1 & 1\\
 & 87937b2 & - & - & - & - & - & - & - & - & - & - & -\\
 & 09ef69c & - & - & - & - & - & - & - & - & - & - & -\\
 & 3fadfdd & 1 & 1 & - & 2 & 3 & 3 & 2 & 1 & - & - & 1\\
 & e7d16c2 & 3 & - & 1 & - & - & 1 & 1 & - & 1 & 1 & 1\\
 & 50ce8c4 & 61 & 61 & 63 & 62 & 57 & 58 & 60 & 61 & 62 & 63 & 61\\
 & 2e9f3a8 & - & - & - & - & - & - & - & - & - & - & -\\
 & c8e61af & - & - & - & - & - & - & - & - & - & - & -\\
 & d8ec011 & - & - & - & - & - & - & - & - & - & - & -\\
 & 7d061e3 & - & - & - & - & - & - & - & - & - & - & -\\
\hline
\multirow{11}{*}{\rotvertical{gson}}
 & b1fb9ca & - & - & - & - & - & - & - & - & - & - & -\\
 & 7a9fd59 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7\\
 & 03a72e7 & - & - & - & - & - & - & - & - & - & 0 & 3\\
 & 74e3711 & - & - & - & - & - & - & - & - & - & - & -\\
 & ada597e & - & - & - & - & - & - & - & - & - & - & -\\
 & a300148 & - & - & - & - & - & - & - & - & - & - & -\\
 & 9a24219 & - & - & - & - & - & - & - & - & - & - & -\\
 & 9e6f2ba & - & - & - & - & - & - & - & - & - & - & -\\
 & 44cad04 & 4 & 5 & 4 & 6 & 4 & 4 & 4 & 4 & 4 & 3 & 5\\
 & b2c00a3 & - & - & - & - & - & - & - & - & - & - & -\\
\hline
\multirow{11}{*}{\rotvertical{jsoup}}
 & 426ffe7 & 126 & 125 & 125 & 123 & 126 & 126 & 127 & 123 & 121 & 119 & 121\\
 & a810d2e & - & - & - & - & - & - & - & - & - & - & -\\
 & 6be19a6 & - & - & - & - & - & - & - & - & - & - & -\\
 & e38dfd4 & - & - & - & - & - & - & - & - & - & - & -\\
 & e9feec9 & - & - & - & - & - & - & 1 & - & 1 & - & -\\
 & 0f7e0cc & 1 & - & - & 1 & 1 & - & 1 & 1 & - & 1 & -\\
 & 2c4e79b & - & - & - & - & - & - & - & - & - & - & -\\
 & e5210d1 & - & - & - & - & - & - & - & - & - & - & -\\
 & df272b7 & - & - & - & - & - & - & - & - & - & - & -\\
 & 3676b13 & 3 & 3 & 6 & 2 & 3 & 4 & 1 & 1 & 1 & 1 & -\\
\hline
\multirow{11}{*}{\rotvertical{mustache.java}}
 & a1197f7 & 28 & 22 & - & - & - & - & - & - & - & - & -\\
 & 8877027 & - & - & - & - & - & - & - & - & - & - & -\\
 & d8936b4 & - & - & - & - & - & - & - & - & - & - & -\\
 & 88718bc & 13 & 12 & 11 & 13 & 13 & 11 & 13 & 12 & 12 & 12 & 12\\
 & 339161f & 143 & 135 & 146 & - & - & - & - & 138 & - & - & 144\\
 & 774ae7a & 18 & 23 & 18 & 3 & 17 & 18 & 15 & 16 & 19 & 17 & 20\\
 & 94847cc & 122 & - & - & 112 & - & 61 & 72 & 57 & 40 & 42 & 37\\
 & eca08ca & - & - & - & - & - & - & - & - & - & - & -\\
 & 6d7225c & - & - & - & - & - & - & - & - & - & - & -\\
 & 8ac71b7 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2\\
\hline
\multirow{11}{*}{\rotvertical{xwiki-commons}}
 & ffc3997 & - & - & - & - & - & - & - & - & - & - & -\\
 & ced2635 & - & - & - & - & - & - & - & - & - & - & -\\
 & 10841b1 & - & - & - & - & - & - & - & - & - & - & -\\
 & 848c984 & - & - & - & - & - & - & - & - & - & - & -\\
 & adfefec & 22 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
 & d3101ae & 9 & 18 & 15 & 13 & 14 & 15 & 14 & - & 15 & 12 & 15\\
 & a0e8b77 & 10 & 19 & - & 14 & 15 & 17 & 15 & 16 & 16 & 13 & 16\\
 & 78ff099 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4\\
 & 1b79714 & - & - & - & - & - & - & - & - & - & - & -\\
 & 6dc9059 & - & - & - & - & - & - & - & - & - & - & -\\
\hline
